The TESS Grand Unified Hot Jupiter Survey. III. Thirty More Giant Planets

We present the discovery of 30 transiting giant planets that were initially detected using data from NASA's Transiting Exoplanet Survey Satellite (TESS) mission. These new planets orbit relatively bright ($G \leq 12.5$) FGK host stars with orbital periods between 1.6 and 8.2 days, and have radii between 0.9 and 1.7 Jupiter radii. We performed follow-up ground-based photometry, high angular-resolution imaging, high-resolution spectroscopy and radial velocity monitoring for each of these objects to confirm that they are planets and determine their masses and other system parameters. The planets' masses span more than an order of magnitude ($0.17\,M_J < M_p < 3.3\,M_J$). For two planets, TOI-3593 b and TOI-4961 b, we measured significant non-zero eccentricities of $0.11^{+0.05}_{-0.03}$ and $0.18^{+0.04}_{-0.05}$ respectively, while for the other planets, the data typically provide a 1-$\sigma$ upper bound of 0.15 on the eccentricity. These discoveries represent a major step toward assembling a complete, magnitude-limited sample of transiting hot Jupiters around FGK stars.

==> catalog_props_0.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-2031} & \colhead{TOI-2169} & \colhead{TOI-2346} & \colhead{TOI-2382} & \colhead{TOI-2876} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 470127886 & 8516795 & 317483660 & 2760219 & 10827386 &  \\
Gaia DR3 & 2299101254886404608 & 4535299582687857920 & 2996776253547606656 & 2418732758551062272 & 2929750922377138816 &  \\
2MASS & 22042815+8133572 & 18364082+2315315 & 05522231-1322209 & 23453002-1606509 & 07205934-2106527 &  \\
WISE & J220428.23+813357.3 & J183640.83+231531.0 & J055222.30-132220.9 & J234530.03-160650.8 & J072059.35-210652.6 &  \\
UCAC4 & 858-013103 & 567-067568 & 384-010383 & 370-190011 & 345-026713 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 22:04:28.280 & 18:36:40.827 & 05:52:22.297 & 23:45:30.045 & 07:20:59.347 & 1 \\
Decl. (J2000) & +81:33:57.42 & +23:15:31.01 & -13:22:20.89 & -16:06:50.85 & -21:06:52.74 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $25.790\pm 0.017$ & $5.505\pm 0.012$ & $-11.225\pm 0.014$ & $12.372\pm 0.015$ & $15.534\pm 0.034$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $2.398\pm 0.014$ & $-31.042\pm 0.016$ & $3.109\pm 0.015$ & $-5.571\pm 0.012$ & $2.554\pm 0.046$ & 1 \\
Parallax (mas) & $3.618\pm 0.013$ & $2.779\pm 0.017$ & $2.292\pm 0.016$ & $2.355\pm 0.016$ & $4.520\pm 0.011$ & 1 \\
$b$ ($^{\circ}$) & 20.711 & 13.455 & -19.035 & -71.162 & -3.297 & 1 \\
$l$ ($^{\circ}$) & 116.940 & 52.422 & 218.564 & 65.339 & 235.013 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $10.761\pm 0.036$ & $10.553\pm 0.006$ & $11.558\pm 0.017$ & $11.441\pm 0.006$ & $11.704\pm 0.006$ & 2 \\
$G$ (mag) & $11.112\pm 0.003$ & $10.959\pm 0.003$ & $11.917\pm 0.003$ & $11.847\pm 0.003$ & $12.248\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $11.367\pm 0.003$ & $11.255\pm 0.003$ & $12.184\pm 0.003$ & $12.154\pm 0.003$ & $12.696\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $10.700\pm 0.004$ & $10.495\pm 0.004$ & $11.490\pm 0.004$ & $11.381\pm 0.004$ & $11.641\pm 0.004$ & 1 \\
$B$ (mag) & $11.691\pm 0.010$ & -- & $12.556\pm 0.030$ & $12.599\pm 0.040$ & $13.384\pm 0.020$ & 3 \\
$V$ (mag) & $11.226\pm 0.010$ & -- & $12.012\pm 0.040$ & $11.969\pm 0.050$ & $12.455\pm 0.020$ & 3 \\
$g$ (mag) & $11.382\pm 0.010$ & -- & $12.237\pm 0.030$ & $12.223\pm 0.010$ & $12.889\pm 0.020$ & 3 \\
$r$ (mag) & $11.114\pm 0.010$ & -- & $11.884\pm 0.050$ & $11.823\pm 0.010$ & $12.174\pm 0.040$ & 3 \\
$i$ (mag) & -- & -- & $11.772\pm 0.080$ & $11.708\pm 0.020$ & $12.001\pm 0.100$ & 3 \\
$J$ (mag) & $10.312\pm 0.026$ & $10.008\pm 0.025$ & $11.001\pm 0.022$ & $10.885\pm 0.022$ & $10.937\pm 0.022$ & 4 \\
$H$ (mag) & $10.011\pm 0.031$ & $9.734\pm 0.019$ & $10.809\pm 0.026$ & $10.628\pm 0.021$ & $10.550\pm 0.024$ & 4 \\
$K_s$ (mag) & $9.971\pm 0.023$ & $9.669\pm 0.016$ & $10.712\pm 0.019$ & $10.578\pm 0.023$ & $10.443\pm 0.023$ & 4 \\
$W1$ (mag) & $9.922\pm 0.023$ & $9.647\pm 0.023$ & $10.703\pm 0.022$ & $10.515\pm 0.023$ & $10.379\pm 0.022$ & 5 \\
$W2$ (mag) & $9.948\pm 0.021$ & $9.671\pm 0.021$ & $10.708\pm 0.020$ & $10.581\pm 0.021$ & $10.485\pm 0.020$ & 5 \\
$W3$ (mag) & $9.872\pm 0.033$ & $9.636\pm 0.046$ & $10.643\pm 0.098$ & $10.488\pm 0.085$ & $10.325\pm 0.058$ & 5%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> catalog_props_1.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-2886} & \colhead{TOI-2986} & \colhead{TOI-2992} & \colhead{TOI-3135} & \colhead{TOI-3160} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 318796593 & 148497855 & 49045066 & 448098793 & 440872576 &  \\
Gaia DR3 & 3046930579529070464 & 3764588660860363264 & 5450366519997969536 & 5847114914267582848 & 6225252356194921728 &  \\
2MASS & 07200185-1034112 & 10550519-0628424 & 10571599-3219209 & 13512628-6946211 & 14581582-2740572 &  \\
WISE & J072001.84-103411.4 & J105505.17-062842.3 & J105715.98-321920.8 & J135126.23-694621.2 & J145815.81-274057.1 &  \\
UCAC4 & 398-025129 & 418-053487 & 289-060621 & 102-067287 & 312-076853 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 07:20:01.847 & 10:55:05.174 & 10:57:15.975 & 13:51:26.213 & 14:58:15.805 & 1 \\
Decl. (J2000) & -10:34:11.36 & -06:28:42.43 & -32:19:20.77 & -69:46:21.24 & -27:40:57.18 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $-8.364\pm 0.059$ & $-12.960\pm 0.019$ & $-10.117\pm 0.011$ & $-20.966\pm 0.010$ & $-13.470\pm 0.038$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $-4.851\pm 0.052$ & $-4.604\pm 0.015$ & $14.805\pm 0.011$ & $-16.628\pm 0.012$ & $1.925\pm 0.035$ & 1 \\
Parallax (mas) & $2.422\pm 0.018$ & $1.806\pm 0.018$ & $1.803\pm 0.013$ & $4.560\pm 0.012$ & $2.048\pm 0.037$ & 1 \\
$b$ ($^{\circ}$) & 1.445 & 46.164 & 24.637 & -7.506 & 27.300 & 1 \\
$l$ ($^{\circ}$) & 225.588 & 258.710 & 276.559 & 308.110 & 334.516 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $11.786\pm 0.006$ & $12.068\pm 0.007$ & $11.973\pm 0.006$ & $11.099\pm 0.006$ & $11.933\pm 0.007$ & 2 \\
$G$ (mag) & $12.187\pm 0.003$ & $12.467\pm 0.003$ & $12.380\pm 0.003$ & $11.575\pm 0.003$ & $12.366\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $12.490\pm 0.003$ & $12.767\pm 0.003$ & $12.690\pm 0.003$ & $11.944\pm 0.003$ & $12.688\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $11.721\pm 0.004$ & $12.003\pm 0.004$ & $11.905\pm 0.004$ & $11.036\pm 0.004$ & $11.860\pm 0.004$ & 1 \\
$B$ (mag) & -- & $13.210\pm 0.040$ & $13.143\pm 0.010$ & $12.389\pm 0.010$ & $13.113\pm 0.000$ & 3 \\
$V$ (mag) & -- & $12.609\pm 0.030$ & $12.547\pm 0.040$ & $11.699\pm 0.010$ & $12.516\pm 0.030$ & 3 \\
$g$ (mag) & -- & $12.869\pm 0.020$ & $12.789\pm 0.010$ & $12.060\pm 0.070$ & $12.774\pm 0.010$ & 3 \\
$r$ (mag) & -- & $12.460\pm 0.020$ & $12.362\pm 0.030$ & $11.508\pm 0.080$ & $12.365\pm 0.060$ & 3 \\
$i$ (mag) & -- & $12.371\pm 0.040$ & $12.230\pm 0.090$ & $11.316\pm 0.010$ & $12.184\pm 0.030$ & 3 \\
$J$ (mag) & $11.206\pm 0.024$ & $11.518\pm 0.022$ & $11.356\pm 0.022$ & $10.443\pm 0.023$ & $11.287\pm 0.024$ & 4 \\
$H$ (mag) & $10.977\pm 0.026$ & $11.216\pm 0.022$ & $11.092\pm 0.021$ & $10.052\pm 0.021$ & $11.004\pm 0.026$ & 4 \\
$K_s$ (mag) & $10.918\pm 0.025$ & $11.187\pm 0.019$ & $11.027\pm 0.022$ & $10.009\pm 0.021$ & $10.894\pm 0.019$ & 4 \\
$W1$ (mag) & $10.853\pm 0.024$ & $11.134\pm 0.023$ & $10.999\pm 0.024$ & $9.959\pm 0.023$ & $10.819\pm 0.022$ & 5 \\
$W2$ (mag) & $10.892\pm 0.024$ & $11.189\pm 0.021$ & $11.030\pm 0.021$ & $9.991\pm 0.020$ & $10.857\pm 0.021$ & 5 \\
$W3$ (mag) & $10.890\pm 0.130$ & $11.046\pm 0.131$ & $10.988\pm 0.118$ & $10.006\pm 0.050$ & $10.812\pm 0.133$ & 5%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> catalog_props_2.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-3464} & \colhead{TOI-3474} & \colhead{TOI-3486} & \colhead{TOI-3523} & \colhead{TOI-3593} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 290504044 & 274367763 & 221861843 & 417047499 & 162289289 &  \\
Gaia DR3 & 5989042791436795648 & 5986650013613194624 & 5927041953543630592 & 2080811118319262080 & 1900293230549817856 &  \\
2MASS & 15375593-4447237 & 15340081-4757491 & 16374641-5918171 & 20170801+4254236 & 22060153+3412422 &  \\
WISE & J153755.92-444723.7 & J153400.81-475749.2 & J163746.38-591817.9 & J201708.01+425423.4 & J220601.52+341242.0 &  \\
UCAC4 & 227-094692 & 211-109202 & 154-187707 & 665-088063 & 622-124124 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 15:37:55.923 & 15:34:00.803 & 16:37:46.367 & 20:17:08.030 & 22:06:01.527 & 1 \\
Decl. (J2000) & -44:47:23.73 & -47:57:49.18 & -59:18:18.42 & +42:54:23.52 & +34:12:41.96 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $3.716\pm 0.082$ & $-8.577\pm 0.016$ & $-25.419\pm 0.012$ & $0.651\pm 0.031$ & $0.306\pm 0.012$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $-11.814\pm 0.061$ & $-2.191\pm 0.014$ & $-73.423\pm 0.011$ & $-12.392\pm 0.034$ & $-21.443\pm 0.016$ & 1 \\
Parallax (mas) & $1.708\pm 0.013$ & $2.424\pm 0.014$ & $6.500\pm 0.011$ & $1.651\pm 0.029$ & $4.454\pm 0.016$ & 1 \\
$b$ ($^{\circ}$) & 8.679 & 6.518 & -8.158 & 4.147 & -17.223 & 1 \\
$l$ ($^{\circ}$) & 331.413 & 328.971 & 328.427 & 79.803 & 88.040 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $12.072\pm 0.006$ & $11.967\pm 0.006$ & $11.487\pm 0.006$ & $12.104\pm 0.022$ & $11.488\pm 0.006$ & 2 \\
$G$ (mag) & $12.499\pm 0.003$ & $12.432\pm 0.003$ & $12.107\pm 0.003$ & $12.497\pm 0.003$ & $12.025\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $12.829\pm 0.003$ & $12.797\pm 0.003$ & $12.642\pm 0.003$ & $12.758\pm 0.003$ & $12.464\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $12.002\pm 0.004$ & $11.904\pm 0.004$ & $11.424\pm 0.004$ & $12.017\pm 0.004$ & $11.427\pm 0.004$ & 1 \\
$B$ (mag) & $13.291\pm 0.010$ & $13.311\pm 0.010$ & $13.470\pm 0.010$ & $13.245\pm 0.010$ & $13.112\pm 0.030$ & 3 \\
$V$ (mag) & $12.629\pm 0.010$ & $12.659\pm 0.010$ & $12.446\pm 0.010$ & $12.763\pm 0.010$ & $12.190\pm 0.040$ & 3 \\
$g$ (mag) & $12.964\pm 0.010$ & -- & $12.925\pm 0.010$ & $12.897\pm 0.010$ & $12.621\pm 0.030$ & 3 \\
$r$ (mag) & $12.460\pm 0.040$ & -- & $12.065\pm 0.010$ & $12.779\pm 0.010$ & $11.919\pm 0.030$ & 3 \\
$i$ (mag) & $12.264\pm 0.040$ & -- & $11.781\pm 0.010$ & -- & $11.675\pm 0.030$ & 3 \\
$J$ (mag) & $11.413\pm 0.044$ & $11.282\pm 0.022$ & $10.601\pm 0.023$ & $11.449\pm 0.023$ & $10.730\pm 0.021$ & 4 \\
$H$ (mag) & $11.118\pm 0.025$ & $10.973\pm 0.023$ & $10.131\pm 0.025$ & $11.230\pm 0.032$ & $10.379\pm 0.017$ & 4 \\
$K_s$ (mag) & $11.095\pm 0.036$ & $10.943\pm 0.025$ & $10.004\pm 0.021$ & $11.146\pm 0.023$ & $10.266\pm 0.015$ & 4 \\
$W1$ (mag) & $10.996\pm 0.024$ & $10.845\pm 0.023$ & $9.949\pm 0.023$ & $11.025\pm 0.023$ & $10.225\pm 0.023$ & 5 \\
$W2$ (mag) & $11.037\pm 0.022$ & $10.891\pm 0.022$ & $10.029\pm 0.020$ & $11.076\pm 0.021$ & $10.289\pm 0.021$ & 5 \\
$W3$ (mag) & $11.215\pm 0.164$ & $11.079\pm 0.119$ & $9.974\pm 0.061$ & $10.501\pm 0.193$ & $10.273\pm 0.059$ & 5%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> catalog_props_3.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-3682} & \colhead{TOI-3856} & \colhead{TOI-3877} & \colhead{TOI-3980} & \colhead{TOI-4214} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 28961316 & 125552076 & 144310492 & 312548829 & 409594381 &  \\
Gaia DR3 & 117190351631297152 & 647864446160474624 & 759209995840837248 & 426758571995216768 & 3032656414642552192 &  \\
2MASS & 03210600+2517505 & 09405353+2757006 & 11214909+3359291 & 00512203+5934330 & 07205987-1355343 &  \\
WISE & J032106.04+251750.2 & J094053.51+275700.6 & J112149.08+335928.9 & J005122.05+593433.0 & J072059.88-135534.5 &  \\
UCAC4 & 577-007481 & 590-047477 & 620-047600 & 748-007931 & 381-029686 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 03:21:06.056 & 09:40:53.501 & 11:21:49.073 & 00:51:22.066 & 07:20:59.879 & 1 \\
Decl. (J2000) & +25:17:50.15 & +27:57:00.57 & +33:59:28.97 & +59:34:33.10 & -13:55:34.33 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $34.818\pm 0.023$ & $-21.061\pm 0.014$ & $-20.033\pm 0.012$ & $17.139\pm 0.008$ & $-0.331\pm 0.073$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $-18.553\pm 0.015$ & $-5.487\pm 0.011$ & $-3.630\pm 0.013$ & $2.820\pm 0.010$ & $-15.227\pm 0.060$ & 1 \\
Parallax (mas) & $2.559\pm 0.017$ & $3.232\pm 0.014$ & $2.035\pm 0.016$ & $2.023\pm 0.011$ & $2.959\pm 0.017$ & 1 \\
$b$ ($^{\circ}$) & -26.374 & 48.028 & 69.575 & -3.296 & 0.078 & 1 \\
$l$ ($^{\circ}$) & 160.750 & 200.346 & 187.832 & 122.923 & 228.663 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $11.319\pm 0.007$ & $11.655\pm 0.007$ & $11.912\pm 0.007$ & $11.863\pm 0.006$ & $11.007\pm 0.006$ & 2 \\
$G$ (mag) & $11.869\pm 0.003$ & $12.122\pm 0.003$ & $12.357\pm 0.003$ & $12.364\pm 0.003$ & $11.453\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $12.315\pm 0.003$ & $12.491\pm 0.003$ & $12.696\pm 0.003$ & $12.765\pm 0.003$ & $11.794\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $11.257\pm 0.004$ & $11.595\pm 0.004$ & $11.851\pm 0.004$ & $11.797\pm 0.004$ & $10.946\pm 0.004$ & 1 \\
$B$ (mag) & $12.931\pm 0.040$ & $13.032\pm 0.070$ & $13.205\pm 0.000$ & $13.403\pm 0.010$ & $12.318\pm 0.030$ & 3 \\
$V$ (mag) & $12.055\pm 0.070$ & $12.306\pm 0.040$ & $12.480\pm 0.070$ & $12.580\pm 0.010$ & $11.612\pm 0.050$ & 3 \\
$g$ (mag) & $12.497\pm 0.050$ & $12.588\pm 0.050$ & $12.807\pm 0.020$ & $12.911\pm 0.010$ & $11.921\pm 0.040$ & 3 \\
$r$ (mag) & $11.790\pm 0.050$ & $12.038\pm 0.010$ & $12.335\pm 0.060$ & $12.376\pm 0.010$ & $11.442\pm 0.060$ & 3 \\
$i$ (mag) & $11.544\pm 0.050$ & $11.872\pm 0.020$ & $12.288\pm 0.180$ & $12.120\pm 0.010$ & $11.309\pm 0.010$ & 3 \\
$J$ (mag) & $10.533\pm 0.026$ & $11.006\pm 0.023$ & $11.313\pm 0.022$ & $11.133\pm 0.018$ & $10.349\pm 0.022$ & 4 \\
$H$ (mag) & $10.164\pm 0.022$ & $10.693\pm 0.023$ & $11.006\pm 0.022$ & $10.818\pm 0.020$ & $10.096\pm 0.022$ & 4 \\
$K_s$ (mag) & $10.062\pm 0.021$ & $10.611\pm 0.017$ & $10.916\pm 0.018$ & $10.741\pm 0.023$ & $10.036\pm 0.024$ & 4 \\
$W1$ (mag) & $10.033\pm 0.022$ & $10.602\pm 0.023$ & $10.899\pm 0.023$ & $10.663\pm 0.023$ & $10.000\pm 0.022$ & 5 \\
$W2$ (mag) & $10.078\pm 0.020$ & $10.644\pm 0.021$ & $10.939\pm 0.021$ & $10.714\pm 0.021$ & $10.042\pm 0.020$ & 5 \\
$W3$ (mag) & $10.052\pm 0.063$ & $10.602\pm 0.105$ & $10.863\pm 0.102$ & $10.295\pm 0.097$ & $10.098\pm 0.062$ & 5%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> catalog_props_4.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-4487} & \colhead{TOI-4734} & \colhead{TOI-4794} & \colhead{TOI-4961} & \colhead{TOI-5181} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 193754373 & 97714451 & 95589845 & 420202798 & 346667887 &  \\
Gaia DR3 & 2083061376251298688 & 3343402074506386176 & 3034394776886475520 & 6056675572727076736 & 4531901709506539776 &  \\
2MASS & 20254129+4558158 & 06012595+1232525 & 07215606-1233556 & 12500043-5953306 & 18424258+2141593 &  \\
WISE & J202541.29+455815.7 & J060125.95+123252.4 & J072156.05-123355.7 & J125000.44-595330.9 & J184242.59+214159.2 &  \\
UCAC4 & 680-082625 & 513-018751 & 388-028548 & 151-114136 & 559-074776 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 20:25:41.300 & 06:01:25.949 & 07:21:56.068 & 12:50:00.441 & 18:42:42.594 & 1 \\
Decl. (J2000) & +45:58:15.70 & +12:32:52.37 & -12:33:55.68 & -59:53:30.69 & +21:41:59.35 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $-0.573\pm 0.010$ & $-1.768\pm 0.020$ & $-14.434\pm 0.053$ & $2.975\pm 0.040$ & $8.348\pm 0.009$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $-13.497\pm 0.010$ & $-5.118\pm 0.016$ & $-2.603\pm 0.048$ & $-17.996\pm 0.042$ & $2.698\pm 0.012$ & 1 \\
Parallax (mas) & $2.097\pm 0.009$ & $1.685\pm 0.014$ & $1.824\pm 0.015$ & $4.680\pm 0.011$ & $2.090\pm 0.014$ & 1 \\
$b$ ($^{\circ}$) & 4.622 & -5.105 & 0.919 & 2.979 & 11.542 & 1 \\
$l$ ($^{\circ}$) & 83.203 & 196.023 & 227.569 & 302.752 & 51.558 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $11.492\pm 0.016$ & $11.904\pm 0.014$ & $12.047\pm 0.014$ & $11.660\pm 0.006$ & $11.724\pm 0.009$ & 2 \\
$G$ (mag) & $11.920\pm 0.003$ & $12.371\pm 0.003$ & $12.440\pm 0.003$ & $12.260\pm 0.003$ & $17.289\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $12.247\pm 0.003$ & $12.736\pm 0.003$ & $12.738\pm 0.003$ & $12.765\pm 0.003$ & $12.591\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $11.428\pm 0.004$ & $11.843\pm 0.004$ & $11.978\pm 0.004$ & $11.594\pm 0.004$ & $11.656\pm 0.004$ & 1 \\
$B$ (mag) & $12.846\pm 0.010$ & $13.247\pm 0.020$ & $13.280\pm 0.130$ & $13.432\pm 0.060$ & -- & 3 \\
$V$ (mag) & $12.144\pm 0.010$ & $12.552\pm 0.020$ & $12.703\pm 0.170$ & $12.497\pm 0.040$ & -- & 3 \\
$g$ (mag) & $12.391\pm 0.030$ & $12.832\pm 0.020$ & $12.936\pm 0.140$ & $12.925\pm 0.050$ & -- & 3 \\
$r$ (mag) & $11.932\pm 0.010$ & $12.370\pm 0.040$ & $12.525\pm 0.130$ & $12.173\pm 0.040$ & -- & 3 \\
$i$ (mag) & -- & $12.138\pm 0.060$ & $12.349\pm 0.070$ & $11.843\pm 0.030$ & -- & 3 \\
$J$ (mag) & $10.864\pm 0.020$ & $11.224\pm 0.023$ & $11.427\pm 0.022$ & $10.790\pm 0.023$ & $11.026\pm 0.020$ & 4 \\
$H$ (mag) & $10.619\pm 0.021$ & $10.929\pm 0.022$ & $11.188\pm 0.025$ & $10.390\pm 0.022$ & $10.701\pm 0.022$ & 4 \\
$K_s$ (mag) & $10.556\pm 0.014$ & $10.848\pm 0.018$ & $11.123\pm 0.025$ & $10.304\pm 0.023$ & $10.627\pm 0.017$ & 4 \\
$W1$ (mag) & $10.477\pm 0.022$ & $10.829\pm 0.023$ & $11.043\pm 0.022$ & $10.191\pm 0.022$ & $10.528\pm 0.023$ & 5 \\
$W2$ (mag) & $10.519\pm 0.020$ & $10.882\pm 0.020$ & $11.080\pm 0.021$ & $10.255\pm 0.020$ & $10.557\pm 0.020$ & 5 \\
$W3$ (mag) & $10.509\pm 0.069$ & $10.880\pm 0.129$ & $11.042\pm 0.125$ & $10.546\pm 0.056$ & $10.487\pm 0.080$ & 5%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> catalog_props_5.tex <==
\tablecolumns{7}
\tablehead{
\colhead{\textbf{Target}} & \colhead{TOI-5210} & \colhead{TOI-5322} & \colhead{TOI-5340} & \colhead{TOI-5386} & \colhead{TOI-5592} & \colhead{Source}
}
\startdata
\multicolumn{7}{l}{\textbf{Identifiers}} \\
TIC & 265979849 & 336691874 & 14156936 & 202425357 & 88529975 &  \\
Gaia DR3 & 1838769198425933568 & 2780169409154216448 & 65315118156520320 & 1616054670018575872 & 1101653957463314688 &  \\
2MASS & 20571603+2157007 & 00260704+1420109 & 03571426+2222422 & 15042568+6032101 & 07064320+6551262 &  \\
WISE & J205716.05+215700.7 & J002607.04+142011.1 & J035714.27+222242.0 & J150425.66+603210.4 & J070643.20+655126.1 &  \\
UCAC4 & 560-129377 & 522-000694 & 562-008479 & 753-050776 & 780-019950 &  \\
\multicolumn{7}{l}{\textbf{Astrometric Measurements}} \\
R.A. (J2000) & 20:57:16.062 & 00:26:07.041 & 03:57:14.264 & 15:04:25.660 & 07:06:43.204 & 1 \\
Decl. (J2000) & +21:57:00.74 & +14:20:11.15 & +22:22:42.19 & +60:32:10.44 & +65:51:26.26 & 1 \\
$\mu_{\alpha}$ (mas yr$^{-1}$) & $23.346\pm 0.018$ & $-10.905\pm 0.020$ & $10.228\pm 0.072$ & $-16.116\pm 0.029$ & $5.096\pm 0.026$ & 1 \\
$\mu_{\delta}$ (mas yr$^{-1}$) & $3.362\pm 0.016$ & $6.457\pm 0.016$ & $-11.137\pm 0.044$ & $6.295\pm 0.028$ & $-10.573\pm 0.034$ & 1 \\
Parallax (mas) & $3.297\pm 0.017$ & $2.067\pm 0.018$ & $1.887\pm 0.013$ & $2.608\pm 0.024$ & $1.704\pm 0.012$ & 1 \\
$b$ ($^{\circ}$) & -15.090 & -48.082 & -23.167 & 49.740 & 26.126 & 1 \\
$l$ ($^{\circ}$) & 67.902 & 113.731 & 169.732 & 98.269 & 149.968 & 1 \\
\multicolumn{7}{l}{\textbf{Photometric Measurements}} \\
$T$ (mag) & $11.419\pm 0.006$ & $12.007\pm 0.007$ & $11.708\pm 0.009$ & $11.350\pm 0.007$ & $12.136\pm 0.007$ & 2 \\
$G$ (mag) & $11.932\pm 0.003$ & $12.471\pm 0.003$ & $12.198\pm 0.003$ & $11.756\pm 0.003$ & $12.485\pm 0.003$ & 1 \\
$G_\mathrm{BP}$ (mag) & $12.340\pm 0.003$ & $12.839\pm 0.003$ & $12.586\pm 0.003$ & $12.056\pm 0.003$ & $12.747\pm 0.003$ & 1 \\
$G_\mathrm{RP}$ (mag) & $11.356\pm 0.004$ & $11.936\pm 0.004$ & $11.639\pm 0.004$ & $11.288\pm 0.004$ & $12.071\pm 0.004$ & 1 \\
$B$ (mag) & -- & $13.359\pm 0.040$ & $13.123\pm 0.020$ & $12.545\pm 0.040$ & $13.189\pm 0.060$ & 3 \\
$V$ (mag) & -- & $12.651\pm 0.010$ & $12.432\pm 0.030$ & $11.836\pm 0.040$ & $12.586\pm 0.050$ & 3 \\
$g$ (mag) & -- & $12.981\pm 0.040$ & $12.700\pm 0.070$ & $12.180\pm 0.040$ & $12.877\pm 0.040$ & 3 \\
$r$ (mag) & -- & $12.440\pm 0.010$ & $12.211\pm 0.030$ & $11.683\pm 0.050$ & $12.453\pm 0.070$ & 3 \\
$i$ (mag) & -- & $12.226\pm 0.050$ & $13.599\pm 0.900$ & $11.541\pm 0.060$ & $12.392\pm 0.050$ & 3 \\
$J$ (mag) & $10.683\pm 0.025$ & $11.301\pm 0.027$ & $10.945\pm 0.024$ & $10.768\pm 0.020$ & $11.636\pm 0.023$ & 4 \\
$H$ (mag) & $10.345\pm 0.030$ & $10.950\pm 0.032$ & $10.694\pm 0.027$ & $10.459\pm 0.019$ & $11.413\pm 0.024$ & 4 \\
$K_s$ (mag) & $10.308\pm 0.020$ & $10.900\pm 0.018$ & $10.607\pm 0.027$ & $10.414\pm 0.016$ & $11.363\pm 0.018$ & 4 \\
$W1$ (mag) & $10.277\pm 0.023$ & $10.863\pm 0.024$ & $10.568\pm 0.023$ & $10.384\pm 0.022$ & $11.291\pm 0.024$ & 5 \\
$W2$ (mag) & $10.312\pm 0.020$ & $10.932\pm 0.021$ & $10.594\pm 0.019$ & $10.426\pm 0.019$ & $11.315\pm 0.021$ & 5 \\
$W3$ (mag) & $10.300\pm 0.064$ & $11.001\pm 0.253$ & $10.588\pm 0.098$ & $10.348\pm 0.053$ & $11.426\pm 0.173$ & 5%
\enddata


==> comp_fit_results_0.tex <==
\tablecolumns{6}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-3160B} & \colhead{TOI-3523B} & \colhead{TOI-5181B} & \colhead{TOI-5386B}
}
\startdata
\multicolumn{6}{l}{\textbf{Secondary Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $0.645^{+0.039}_{-0.036}$ & $0.765^{+0.032}_{-0.030}$ & $0.543 \pm 0.025$ & $0.738^{+0.032}_{-0.031}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $0.618^{+0.035}_{-0.034}$ & $0.700^{+0.024}_{-0.023}$ & $0.503 \pm 0.018$ & $0.673^{+0.021}_{-0.020}$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.665^{+0.034}_{-0.033}$ & $4.631 \pm 0.025$ & $4.769 \pm 0.025$ & $4.650 \pm 0.025$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $3.85^{+0.53}_{-0.46}$ & $3.14^{+0.28}_{-0.26}$ & $6.00^{+0.55}_{-0.50}$ & $3.41^{+0.30}_{-0.27}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $0.116^{+0.025}_{-0.016}$ & $0.336^{+0.057}_{-0.047}$ & $0.0491^{+0.0019}_{-0.0021}$ & $0.174^{+0.029}_{-0.024}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $4290^{+160}_{-120}$ & $5260 \pm 180$ & $3828 \pm 71$ & $4550^{+170}_{-160}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $-0.018^{+0.093}_{-0.094}$ & $-0.183^{+0.077}_{-0.083}$ & $0.280^{+0.088}_{-0.084}$ & $0.239^{+0.095}_{-0.092}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{a} & Initial metallicity & $-0.020^{+0.071}_{-0.077}$ & $-0.180^{+0.062}_{-0.068}$ & $0.247^{+0.069}_{-0.066}$ & $0.203^{+0.080}_{-0.077}$ \\
Age (Gyr)\tablenotemark{a} & Stellar age & $5.5^{+2.5}_{-2.0}$ & $4.3^{+1.6}_{-1.1}$ & $4.1^{+1.5}_{-1.1}$ & $3.4^{+1.5}_{-1.2}$ \\
EEP & Equal evolutionary phase & $316^{+11}_{-12}$ & $327.9^{+8.7}_{-9.0}$ & $292.7 \pm 9.3$ & $309^{+11}_{-13}$%
\enddata


==> fit_results_0.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-2031A\,b} & \colhead{TOI-2169A\,b} & \colhead{TOI-2346\,b} & \colhead{TOI-2382\,b/NGTS-37\,b} & \colhead{TOI-2876\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $5.71548654^{+0.00000076}_{-0.00000075}$ & $8.2148282^{+0.0000081}_{-0.0000080}$ & $3.3312029 \pm 0.0000024$ & $4.6612061 \pm 0.0000032$ & $6.2996431 \pm 0.0000070$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2459806.029135 \pm 0.000076$ & $2459732.67384 \pm 0.00050$ & $2459040.83958 \pm 0.00029$ & $2459215.45850^{+0.00044}_{-0.00045}$ & $2459109.77217 \pm 0.00044$ \\
$T_{14}$ (days) & Transit duration & $0.16779 \pm 0.00042$ & $0.1807 \pm 0.0018$ & $0.1582^{+0.0011}_{-0.0010}$ & $0.0946^{+0.0018}_{-0.0017}$ & $0.0937^{+0.0014}_{-0.0013}$ \\
$\tau$ (days) & Ingress/egress duration & $0.01781 \pm 0.00047$ & $0.0249^{+0.0018}_{-0.0017}$ & $0.01568^{+0.00073}_{-0.00045}$ & $0.0415^{+0.0065}_{-0.0072}$ & $0.0220^{+0.0017}_{-0.0015}$ \\
$a/R_\star$ & Planet-star separation & $11.43 \pm 0.13$ & $10.57^{+0.32}_{-0.31}$ & $7.40^{+0.07}_{-0.15}$ & $8.95^{+0.30}_{-0.31}$ & $16.10^{+0.42}_{-0.44}$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.011010^{+0.000067}_{-0.000068}$ & $0.00397 \pm 0.00010$ & $0.01147 \pm 0.00047$ & $0.00628^{+0.00057}_{-0.00031}$ & $0.01025^{+0.00034}_{-0.00032}$ \\
$i$ (deg) & Inclination & $88.32^{+0.19}_{-0.17}$ & $85.80 \pm 0.21$ & $89.01^{+0.69}_{-0.92}$ & $84.11^{+0.24}_{-0.28}$ & $87.13^{+0.12}_{-0.13}$ \\
$K$ (m/s) & RV semi-amplitude & $81 \pm 23$ & $82.5 \pm 5.3$ & $144 \pm 25$ & $76^{+25}_{-26}$ & $19.5 \pm 5.9$ \\
$a$ (AU) & Semimajor axis & $0.0660^{+0.0011}_{-0.0012}$ & $0.0896^{+0.0014}_{-0.0015}$ & $0.04730^{+0.00086}_{-0.00094}$ & $0.0590 \pm 0.0010$ & $0.0654^{+0.0009}_{-0.0011}$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $1.267 \pm 0.024$ & $1.116^{+0.037}_{-0.036}$ & $1.438^{+0.043}_{-0.041}$ & $1.093^{+0.076}_{-0.051}$ & $0.860^{+0.030}_{-0.028}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $0.80 \pm 0.23$ & $1.037^{+0.077}_{-0.076}$ & $1.24 \pm 0.22$ & $0.74 \pm 0.25$ & $0.170 \pm 0.052$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.49 \pm 0.14$ & $0.92^{+0.12}_{-0.11}$ & $0.52 \pm 0.10$ & $0.68^{+0.28}_{-0.26}$ & $0.33^{+0.11}_{-0.10}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $3.09^{+0.11}_{-0.14}$ & $3.314^{+0.044}_{-0.045}$ & $3.173^{+0.074}_{-0.086}$ & $3.17^{+0.14}_{-0.19}$ & $2.76^{+0.12}_{-0.15}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.336^{+0.030}_{-0.035}$ & $0.775^{+0.015}_{-0.017}$ & $0.13^{+0.11}_{-0.09}$ & $0.918^{+0.011}_{-0.009}$ & $0.806 \pm 0.014$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.076$ & $< 0.045$ & $< 0.086$ & $< 0.18$ & $< 0.13$ \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $1.58^{+0.47}_{-0.45}$ & $21.1^{+4.6}_{-3.8}$ & $0.133^{+0.031}_{-0.029}$ & $1.26^{+0.67}_{-0.55}$ & $3.0^{+1.2}_{-1.0}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $0.772^{+0.085}_{-0.062}$ & $0.786^{+0.050}_{-0.048}$ & $1.85^{+0.22}_{-0.18}$ & $0.938^{+0.041}_{-0.037}$ & $0.169^{+0.013}_{-0.010}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1358^{+36}_{-28}$ & $1364 \pm 21$ & $1689^{+47}_{-42}$ & $1426^{+15}_{-14}$ & $929^{+17}_{-15}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.174^{+0.060}_{-0.062}$ & $1.420^{+0.069}_{-0.070}$ & $1.271^{+0.070}_{-0.074}$ & $1.260^{+0.064}_{-0.065}$ & $0.939^{+0.041}_{-0.045}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.241 \pm 0.022$ & $1.820^{+0.047}_{-0.046}$ & $1.380^{+0.027}_{-0.026}$ & $1.417^{+0.041}_{-0.038}$ & $0.873^{+0.021}_{-0.020}$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.320 \pm 0.014$ & $4.069 \pm 0.030$ & $4.265^{+0.014}_{-0.022}$ & $4.235^{+0.033}_{-0.036}$ & $4.529^{+0.025}_{-0.029}$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.865^{+0.031}_{-0.029}$ & $0.331^{+0.031}_{-0.028}$ & $0.689^{+0.020}_{-0.041}$ & $0.624^{+0.064}_{-0.062}$ & $1.99 \pm 0.16$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $2.46^{+0.31}_{-0.20}$ & $4.63^{+0.32}_{-0.31}$ & $3.03^{+0.43}_{-0.35}$ & $2.397^{+0.070}_{-0.069}$ & $0.529^{+0.044}_{-0.034}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $6490^{+170}_{-130}$ & $6270 \pm 130$ & $6480^{+200}_{-180}$ & $6033^{+81}_{-83}$ & $5271^{+110}_{-96}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $-0.24^{+0.09}_{-0.16}$ & $0.123^{+0.076}_{-0.073}$ & $-0.030^{+0.048}_{-0.056}$ & $0.249^{+0.073}_{-0.074}$ & $0.353^{+0.073}_{-0.076}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $-0.12^{+0.07}_{-0.10}$ & $0.217 \pm 0.077$ & $0.081^{+0.046}_{-0.050}$ & $0.287^{+0.064}_{-0.063}$ & $0.318^{+0.071}_{-0.075}$ \\
Age (Gyr) & Stellar age & $2.0^{+1.2}_{-0.9}$ & $2.51^{+0.78}_{-0.65}$ & $1.9^{+1.3}_{-0.9}$ & $3.1^{+1.6}_{-1.3}$ & $3.8^{+4.6}_{-2.7}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $345^{+24}_{-17}$ & $379^{+22}_{-24}$ & $346^{+31}_{-17}$ & $371^{+35}_{-31}$ & $335^{+27}_{-37}$ \\
$A_V$ (mag) & Visual extinction & $0.13^{+0.12}_{-0.09}$ & $0.248^{+0.075}_{-0.081}$ & $0.28 \pm 0.14$ & $0.040^{+0.019}_{-0.025}$ & $0.18^{+0.12}_{-0.10}$ \\
d (pc) & Distance & $276.42^{+0.99}_{-0.98}$ & $359.8 \pm 2.2$ & $436.5^{+3.1}_{-3.0}$ & $424.3 \pm 2.9$ & $221.26 \pm 0.54$%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> fit_results_1.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-2886\,b} & \colhead{TOI-2986\,b} & \colhead{TOI-2992\,b} & \colhead{TOI-3135\,b} & \colhead{TOI-3160A\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $1.60200105^{+0.00000044}_{-0.00000043}$ & $3.2783662^{+0.0000044}_{-0.0000043}$ & $3.0078120 \pm 0.0000019$ & $3.7065585 \pm 0.0000013$ & $3.9712810 \pm 0.0000025$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2459311.01449 \pm 0.00014$ & $2459537.62548^{+0.00072}_{-0.00071}$ & $2459503.55851^{+0.00037}_{-0.00038}$ & $2459595.16441 \pm 0.00018$ & $2459609.98510 \pm 0.00035$ \\
$T_{14}$ (days) & Transit duration & $0.11602^{+0.00070}_{-0.00060}$ & $0.1649^{+0.0017}_{-0.0016}$ & $0.1600^{+0.0016}_{-0.0015}$ & $0.09293^{+0.00086}_{-0.00083}$ & $0.1248 \pm 0.0016$ \\
$\tau$ (days) & Ingress/egress duration & $0.01467^{+0.00073}_{-0.00049}$ & $0.00937^{+0.00056}_{-0.00025}$ & $0.0144^{+0.0014}_{-0.0013}$ & $0.0241 \pm 0.0011$ & $0.0229^{+0.0019}_{-0.0018}$ \\
$a/R_\star$ & Planet-star separation & $4.977^{+0.070}_{-0.099}$ & $6.65^{+0.10}_{-0.17}$ & $6.03 \pm 0.25$ & $10.38 \pm 0.17$ & $8.07^{+0.28}_{-0.27}$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.01897^{+0.00032}_{-0.00031}$ & $0.003415^{+0.000096}_{-0.000095}$ & $0.00666 \pm 0.00013$ & $0.01616^{+0.00038}_{-0.00037}$ & $0.00878^{+0.00022}_{-0.00020}$ \\
$i$ (deg) & Inclination & $87.8^{+1.3}_{-1.1}$ & $88.8^{+0.9}_{-1.2}$ & $86.1^{+1.1}_{-0.9}$ & $85.69 \pm 0.12$ & $84.63 \pm 0.33$ \\
$K$ (m/s) & RV semi-amplitude & $212 \pm 34$ & $38^{+8}_{-11}$ & $414^{+43}_{-45}$ & $130^{+38}_{-34}$ & $144 \pm 17$ \\
$a$ (AU) & Semimajor axis & $0.02871^{+0.00044}_{-0.00051}$ & $0.04489^{+0.00096}_{-0.00088}$ & $0.0434^{+0.0009}_{-0.0013}$ & $0.04756^{+0.00063}_{-0.00073}$ & $0.0505 \pm 0.0012$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $1.663^{+0.041}_{-0.035}$ & $0.829^{+0.023}_{-0.021}$ & $1.227 \pm 0.045$ & $1.218 \pm 0.030$ & $1.228^{+0.046}_{-0.045}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $1.40 \pm 0.23$ & $0.304^{+0.067}_{-0.086}$ & $3.33 \pm 0.39$ & $1.03^{+0.30}_{-0.27}$ & $1.19^{+0.16}_{-0.15}$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.377^{+0.065}_{-0.063}$ & $0.66^{+0.16}_{-0.19}$ & $2.23^{+0.40}_{-0.35}$ & $0.70^{+0.21}_{-0.19}$ & $0.79^{+0.15}_{-0.13}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $3.099^{+0.067}_{-0.078}$ & $3.04^{+0.09}_{-0.14}$ & $3.738^{+0.061}_{-0.065}$ & $3.24^{+0.11}_{-0.13}$ & $3.292^{+0.063}_{-0.067}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.19^{+0.09}_{-0.11}$ & $0.14^{+0.13}_{-0.10}$ & $0.41^{+0.08}_{-0.10}$ & $0.7796^{+0.0092}_{-0.0097}$ & $0.755^{+0.020}_{-0.022}$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.11$ & $< 0.14$ & $< 0.089$ & $< 0.24$ & $< 0.18$ \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $0.00295^{+0.00058}_{-0.00055}$ & $0.43^{+0.12}_{-0.13}$ & $0.48^{+0.14}_{-0.11}$ & $0.35^{+0.12}_{-0.10}$ & $0.54^{+0.14}_{-0.12}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $3.48^{+0.33}_{-0.31}$ & $1.573^{+0.072}_{-0.068}$ & $2.02^{+0.12}_{-0.11}$ & $0.632^{+0.064}_{-0.057}$ & $1.27^{+0.14}_{-0.13}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1978^{+45}_{-46}$ & $1622 \pm 18$ & $1726^{+25}_{-24}$ & $1292^{+31}_{-30}$ & $1539^{+39}_{-40}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.229^{+0.057}_{-0.065}$ & $1.122^{+0.074}_{-0.064}$ & $1.21^{+0.07}_{-0.10}$ & $1.044^{+0.042}_{-0.047}$ & $1.088^{+0.082}_{-0.078}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.241^{+0.024}_{-0.022}$ & $1.458^{+0.033}_{-0.031}$ & $1.545^{+0.046}_{-0.047}$ & $0.985 \pm 0.019$ & $1.346^{+0.042}_{-0.041}$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.340^{+0.015}_{-0.022}$ & $4.165^{+0.018}_{-0.028}$ & $4.139^{+0.042}_{-0.047}$ & $4.469^{+0.016}_{-0.018}$ & $4.217 \pm 0.035$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.908^{+0.039}_{-0.053}$ & $0.517^{+0.023}_{-0.038}$ & $0.457^{+0.059}_{-0.054}$ & $1.537^{+0.079}_{-0.075}$ & $0.629^{+0.067}_{-0.060}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $2.10^{+0.23}_{-0.22}$ & $2.332^{+0.077}_{-0.075}$ & $2.79^{+0.12}_{-0.15}$ & $1.05^{+0.12}_{-0.10}$ & $2.39^{+0.29}_{-0.28}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $6240 \pm 150$ & $5906^{+66}_{-69}$ & $6000^{+100}_{-110}$ & $5890^{+150}_{-140}$ & $6190 \pm 170$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $0.284^{+0.073}_{-0.077}$ & $0.095^{+0.067}_{-0.061}$ & $0.084^{+0.068}_{-0.060}$ & $0.071^{+0.078}_{-0.070}$ & $-0.114^{+0.080}_{-0.095}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $0.270^{+0.067}_{-0.069}$ & $0.152^{+0.059}_{-0.055}$ & $0.149^{+0.065}_{-0.058}$ & $0.055^{+0.075}_{-0.069}$ & $-0.020^{+0.071}_{-0.077}$ \\
Age (Gyr) & Stellar age & $1.7^{+1.7}_{-1.1}$ & $6.3^{+2.0}_{-1.7}$ & $4.6^{+2.5}_{-1.4}$ & $1.8^{+2.1}_{-1.2}$ & $5.5^{+2.5}_{-2.0}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $338^{+32}_{-33}$ & $430^{+11}_{-22}$ & $413^{+31}_{-30}$ & $326^{+21}_{-37}$ & $417^{+16}_{-31}$ \\
$A_V$ (mag) & Visual extinction & $0.33^{+0.12}_{-0.13}$ & $0.043^{+0.024}_{-0.027}$ & $0.167^{+0.045}_{-0.073}$ & $0.29 \pm 0.13$ & $0.25^{+0.12}_{-0.14}$ \\
d (pc) & Distance & $413.7^{+3.1}_{-3.0}$ & $554.4^{+5.3}_{-5.2}$ & $554.5^{+4.2}_{-4.1}$ & $219.28 \pm 0.56$ & $486.6^{+8.7}_{-8.4}$%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> fit_results_2.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-3464\,b} & \colhead{TOI-3474\,b} & \colhead{TOI-3486\,b} & \colhead{TOI-3523A\,b} & \colhead{TOI-3593\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $3.6515568^{+0.0000060}_{-0.0000061}$ & $3.8795105 \pm 0.0000045$ & $2.21778105 \pm 0.00000088$ & $2.30458952 \pm 0.00000082$ & $3.8212867 \pm 0.0000016$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2459703.56516 \pm 0.00080$ & $2459789.28867 \pm 0.00042$ & $2459797.24218 \pm 0.00018$ & $2460417.45562 \pm 0.00014$ & $2460055.72703 \pm 0.00016$ \\
$T_{14}$ (days) & Transit duration & $0.1045^{+0.0027}_{-0.0025}$ & $0.1583^{+0.0012}_{-0.0011}$ & $0.07153^{+0.00076}_{-0.00074}$ & $0.15207^{+0.00064}_{-0.00053}$ & $0.10357^{+0.00088}_{-0.00092}$ \\
$\tau$ (days) & Ingress/egress duration & $0.0296^{+0.0040}_{-0.0032}$ & $0.01556^{+0.00053}_{-0.00032}$ & $0.01493^{+0.00094}_{-0.00087}$ & $0.01446^{+0.00060}_{-0.00036}$ & $0.01152^{+0.00084}_{-0.00096}$ \\
$a/R_\star$ & Planet-star separation & $7.09 \pm 0.29$ & $8.62^{+0.08}_{-0.13}$ & $8.57 \pm 0.19$ & $5.298^{+0.056}_{-0.097}$ & $11.27^{+0.27}_{-0.32}$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.00654^{+0.00034}_{-0.00032}$ & $0.01148^{+0.00034}_{-0.00033}$ & $0.01515^{+0.00046}_{-0.00044}$ & $0.01022^{+0.00020}_{-0.00017}$ & $0.01210^{+0.00028}_{-0.00029}$ \\
$i$ (deg) & Inclination & $82.89^{+0.37}_{-0.40}$ & $89.33^{+0.47}_{-0.69}$ & $85.20 \pm 0.22$ & $88.3^{+1.1}_{-1.0}$ & $88.09^{+0.63}_{-0.37}$ \\
$K$ (m/s) & RV semi-amplitude & $133^{+28}_{-27}$ & $73^{+17}_{-18}$ & $54.5 \pm 9.8$ & $194 \pm 13$ & $230^{+8}_{-13}$ \\
$a$ (AU) & Semimajor axis & $0.0515^{+0.0012}_{-0.0013}$ & $0.0502 \pm 0.0010$ & $0.03138^{+0.00046}_{-0.00043}$ & $0.03559^{+0.00076}_{-0.00084}$ & $0.04810^{+0.00058}_{-0.00070}$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $1.228^{+0.057}_{-0.053}$ & $1.309^{+0.033}_{-0.032}$ & $0.943^{+0.030}_{-0.029}$ & $1.425^{+0.037}_{-0.035}$ & $0.984^{+0.028}_{-0.026}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $1.25^{+0.27}_{-0.26}$ & $0.61^{+0.14}_{-0.15}$ & $0.312^{+0.057}_{-0.056}$ & $1.37^{+0.12}_{-0.11}$ & $1.78^{+0.09}_{-0.13}$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.83^{+0.24}_{-0.20}$ & $0.337^{+0.081}_{-0.084}$ & $0.46^{+0.10}_{-0.09}$ & $0.587 \pm 0.051$ & $2.31^{+0.24}_{-0.26}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $3.31^{+0.10}_{-0.11}$ & $2.95^{+0.09}_{-0.12}$ & $2.939^{+0.079}_{-0.089}$ & $3.223^{+0.042}_{-0.045}$ & $3.658^{+0.032}_{-0.042}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.877^{+0.012}_{-0.013}$ & $0.10^{+0.10}_{-0.07}$ & $0.718^{+0.017}_{-0.018}$ & $0.16^{+0.09}_{-0.10}$ & $0.34^{+0.07}_{-0.12}$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & $0.105^{+0.052}_{-0.028}$ \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.25$ & $< 0.13$ & $< 0.078$ & $< 0.047$ & -- \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $0.45^{+0.18}_{-0.14}$ & $0.185^{+0.049}_{-0.048}$ & $0.0355^{+0.0098}_{-0.0083}$ & $0.0288^{+0.0032}_{-0.0034}$ & $1.70^{+0.35}_{-0.42}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $1.87^{+0.25}_{-0.19}$ & $1.01^{+0.11}_{-0.10}$ & $0.455^{+0.044}_{-0.036}$ & $3.52^{+0.24}_{-0.23}$ & $0.419^{+0.028}_{-0.031}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1693^{+54}_{-45}$ & $1451^{+38}_{-36}$ & $1190^{+28}_{-24}$ & $1984 \pm 33$ & $1170^{+19}_{-22}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.363^{+0.095}_{-0.099}$ & $1.121^{+0.069}_{-0.067}$ & $0.837^{+0.037}_{-0.034}$ & $1.131^{+0.074}_{-0.078}$ & $1.015^{+0.037}_{-0.043}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.560^{+0.046}_{-0.045}$ & $1.256 \pm 0.025$ & $0.788 \pm 0.017$ & $1.448 \pm 0.035$ & $0.918^{+0.024}_{-0.022}$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.185^{+0.042}_{-0.045}$ & $4.292^{+0.014}_{-0.018}$ & $4.569^{+0.023}_{-0.022}$ & $4.171^{+0.015}_{-0.019}$ & $4.519^{+0.022}_{-0.028}$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.504^{+0.065}_{-0.059}$ & $0.804^{+0.023}_{-0.035}$ & $2.42^{+0.17}_{-0.16}$ & $0.529^{+0.017}_{-0.029}$ & $1.85^{+0.14}_{-0.15}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $3.62^{+0.63}_{-0.47}$ & $1.86^{+0.24}_{-0.21}$ & $0.329^{+0.035}_{-0.028}$ & $3.27^{+0.26}_{-0.24}$ & $0.722^{+0.051}_{-0.058}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $6370^{+290}_{-250}$ & $6020^{+170}_{-160}$ & $4930^{+120}_{-110}$ & $6450 \pm 110$ & $5550^{+100}_{-120}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $0.045^{+0.067}_{-0.051}$ & $0.146^{+0.084}_{-0.081}$ & $0.283^{+0.081}_{-0.085}$ & $-0.366^{+0.076}_{-0.081}$ & $0.384^{+0.080}_{-0.084}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $0.174^{+0.062}_{-0.060}$ & $0.180 \pm 0.072$ & $0.258^{+0.079}_{-0.083}$ & $-0.180^{+0.062}_{-0.068}$ & $0.334^{+0.076}_{-0.079}$ \\
Age (Gyr) & Stellar age & $2.1^{+1.5}_{-1.1}$ & $4.7^{+2.3}_{-1.8}$ & $5.8^{+4.8}_{-3.9}$ & $4.3^{+1.6}_{-1.1}$ & $1.8^{+2.9}_{-1.3}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $350^{+46}_{-18}$ & $395^{+21}_{-36}$ & $337^{+15}_{-32}$ & $414^{+16}_{-25}$ & $320^{+27}_{-41}$ \\
$A_V$ (mag) & Visual extinction & $0.48^{+0.19}_{-0.17}$ & $0.48 \pm 0.15$ & $0.28 \pm 0.16$ & $0.198 \pm 0.065$ & $0.30^{+0.10}_{-0.13}$ \\
d (pc) & Distance & $585.1^{+4.6}_{-4.5}$ & $412.9 \pm 2.4$ & $153.85 \pm 0.27$ & $607 \pm 10$ & $224.51 \pm 0.82$%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> fit_results_3.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-3682\,b} & \colhead{TOI-3856\,b} & \colhead{TOI-3877\,b} & \colhead{TOI-3980\,b} & \colhead{TOI-4214\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $3.3462406 \pm 0.0000023$ & $2.04360352 \pm 0.00000094$ & $4.1235960 \pm 0.0000067$ & $3.6089254^{+0.0000030}_{-0.0000031}$ & $3.4913885^{+0.0000033}_{-0.0000032}$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2459692.65921 \pm 0.00029$ & $2459574.66334 \pm 0.00012$ & $2459753.93391^{+0.00078}_{-0.00079}$ & $2459528.89504 \pm 0.00056$ & $2459129.83460 \pm 0.00034$ \\
$T_{14}$ (days) & Transit duration & $0.1740^{+0.0012}_{-0.0011}$ & $0.07605^{+0.00059}_{-0.00057}$ & $0.1160^{+0.0023}_{-0.0021}$ & $0.0983^{+0.0022}_{-0.0021}$ & $0.1356^{+0.0012}_{-0.0011}$ \\
$\tau$ (days) & Ingress/egress duration & $0.0139^{+0.0011}_{-0.0009}$ & $0.02125^{+0.00081}_{-0.00075}$ & $0.0225^{+0.0024}_{-0.0021}$ & $0.0491^{+0.0011}_{-0.0014}$ & $0.01225^{+0.00098}_{-0.00078}$ \\
$a/R_\star$ & Planet-star separation & $5.93^{+0.17}_{-0.20}$ & $6.622 \pm 0.084$ & $7.85 \pm 0.30$ & $6.52^{+0.27}_{-0.35}$ & $7.52^{+0.23}_{-0.26}$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.004576^{+0.000079}_{-0.000074}$ & $0.01397^{+0.00019}_{-0.00018}$ & $0.00550^{+0.00021}_{-0.00020}$ & $0.0067^{+0.0018}_{-0.0005}$ & $0.004663^{+0.000088}_{-0.000085}$ \\
$i$ (deg) & Inclination & $85.51^{+0.66}_{-0.70}$ & $82.94 \pm 0.14$ & $83.97^{+0.34}_{-0.36}$ & $81.95^{+0.40}_{-0.67}$ & $85.77^{+0.42}_{-0.47}$ \\
$K$ (m/s) & RV semi-amplitude & $24.8^{+8.4}_{-9.1}$ & $80 \pm 15$ & $36.1 \pm 7.6$ & $67^{+21}_{-19}$ & $56.2^{+5.4}_{-5.6}$ \\
$a$ (AU) & Semimajor axis & $0.0480^{+0.0006}_{-0.0015}$ & $0.03250^{+0.00044}_{-0.00049}$ & $0.0529^{+0.0010}_{-0.0014}$ & $0.0494^{+0.0010}_{-0.0018}$ & $0.05018^{+0.00077}_{-0.00094}$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $1.142^{+0.036}_{-0.035}$ & $1.213^{+0.025}_{-0.024}$ & $1.042^{+0.044}_{-0.043}$ & $1.29^{+0.20}_{-0.10}$ & $0.953^{+0.032}_{-0.030}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $0.218^{+0.075}_{-0.080}$ & $0.54 \pm 0.10$ & $0.314^{+0.069}_{-0.067}$ & $0.59^{+0.19}_{-0.17}$ & $0.520^{+0.053}_{-0.054}$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.181 \pm 0.067$ & $0.371^{+0.076}_{-0.074}$ & $0.342^{+0.096}_{-0.084}$ & $0.25 \pm 0.14$ & $0.74^{+0.11}_{-0.10}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $2.62^{+0.13}_{-0.17}$ & $2.955^{+0.078}_{-0.094}$ & $2.85^{+0.10}_{-0.11}$ & $2.92^{+0.15}_{-0.22}$ & $3.152^{+0.052}_{-0.057}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.464^{+0.055}_{-0.056}$ & $0.8141^{+0.0059}_{-0.0060}$ & $0.824^{+0.016}_{-0.018}$ & $0.928^{+0.022}_{-0.014}$ & $0.555 \pm 0.041$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.22$ & $< 0.083$ & $< 0.22$ & $< 0.16$ & $< 0.17$ \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $0.075^{+0.033}_{-0.029}$ & $0.0145^{+0.0032}_{-0.0030}$ & $0.39^{+0.15}_{-0.12}$ & $0.076 \pm 0.070$ & $0.56^{+0.12}_{-0.11}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $1.71^{+0.11}_{-0.10}$ & $1.292^{+0.046}_{-0.043}$ & $0.992^{+0.054}_{-0.045}$ & $1.57^{+0.11}_{-0.10}$ & $1.65^{+0.20}_{-0.15}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1657^{+25}_{-24}$ & $1544^{+14}_{-13}$ & $1445^{+19}_{-17}$ & $1621^{+29}_{-28}$ & $1642^{+47}_{-40}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.32^{+0.05}_{-0.12}$ & $1.096^{+0.045}_{-0.049}$ & $1.160^{+0.066}_{-0.089}$ & $1.24^{+0.08}_{-0.13}$ & $1.382^{+0.064}_{-0.076}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.735 \pm 0.045$ & $1.055 \pm 0.017$ & $1.445^{+0.043}_{-0.042}$ & $1.626^{+0.055}_{-0.050}$ & $1.434^{+0.040}_{-0.038}$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.077^{+0.027}_{-0.040}$ & $4.431^{+0.014}_{-0.015}$ & $4.181^{+0.037}_{-0.042}$ & $4.106^{+0.041}_{-0.063}$ & $4.266^{+0.029}_{-0.036}$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.352^{+0.032}_{-0.034}$ & $1.314^{+0.051}_{-0.050}$ & $0.538^{+0.064}_{-0.059}$ & $0.403^{+0.052}_{-0.061}$ & $0.661^{+0.061}_{-0.065}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $2.87^{+0.17}_{-0.16}$ & $1.002 \pm 0.026$ & $2.030^{+0.061}_{-0.059}$ & $2.77^{+0.21}_{-0.19}$ & $3.04^{+0.42}_{-0.34}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $5703^{+100}_{-98}$ & $5622 \pm 50$ & $5731^{+82}_{-81}$ & $5840 \pm 140$ & $6370^{+220}_{-210}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $0.416^{+0.059}_{-0.067}$ & $0.454^{+0.065}_{-0.076}$ & $0.269^{+0.067}_{-0.069}$ & $0.188^{+0.085}_{-0.086}$ & $0.294^{+0.082}_{-0.086}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $0.410^{+0.054}_{-0.063}$ & $0.408^{+0.057}_{-0.070}$ & $0.294 \pm 0.061$ & $0.226 \pm 0.078$ & $0.322^{+0.070}_{-0.073}$ \\
Age (Gyr) & Stellar age & $4.2^{+2.3}_{-0.8}$ & $2.6^{+2.3}_{-1.7}$ & $5.9^{+2.9}_{-1.7}$ & $4.7^{+3.1}_{-1.3}$ & $1.1^{+1.3}_{-0.8}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $409^{+40}_{-17}$ & $342^{+26}_{-30}$ & $424^{+20}_{-26}$ & $416^{+36}_{-28}$ & $328^{+22}_{-37}$ \\
$A_V$ (mag) & Visual extinction & $0.490^{+0.076}_{-0.075}$ & $0.026^{+0.017}_{-0.018}$ & $0.038^{+0.022}_{-0.025}$ & $0.446^{+0.089}_{-0.090}$ & $0.48 \pm 0.15$ \\
d (pc) & Distance & $390.5 \pm 2.6$ & $309.3 \pm 1.4$ & $491.2^{+3.9}_{-3.8}$ & $494.3^{+2.7}_{-2.6}$ & $337.8 \pm 1.9$%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> fit_results_4.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-4487A\,b} & \colhead{TOI-4734\,b} & \colhead{TOI-4794\,b} & \colhead{TOI-4961\,b} & \colhead{TOI-5181A\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $3.9540709 \pm 0.0000021$ & $6.235633^{+0.000010}_{-0.000011}$ & $3.5658116 \pm 0.0000063$ & $7.4791820 \pm 0.0000082$ & $3.8922295 \pm 0.0000023$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2460079.02001 \pm 0.00025$ & $2459710.23803^{+0.00071}_{-0.00073}$ & $2458889.68950^{+0.00071}_{-0.00070}$ & $2459884.82079 \pm 0.00036$ & $2460100.73085^{+0.00033}_{-0.00032}$ \\
$T_{14}$ (days) & Transit duration & $0.1779 \pm 0.0012$ & $0.2422 \pm 0.0018$ & $0.1673 \pm 0.0019$ & $0.1470 \pm 0.0020$ & $0.1227^{+0.0015}_{-0.0014}$ \\
$\tau$ (days) & Ingress/egress duration & $0.0158^{+0.0012}_{-0.0011}$ & $0.01264^{+0.00063}_{-0.00028}$ & $0.0145^{+0.0011}_{-0.0006}$ & $0.0259^{+0.0022}_{-0.0023}$ & $0.0235^{+0.0016}_{-0.0015}$ \\
$a/R_\star$ & Planet-star separation & $7.16^{+0.24}_{-0.23}$ & $8.59^{+0.09}_{-0.19}$ & $7.32^{+0.14}_{-0.25}$ & $17.15^{+0.60}_{-0.61}$ & $7.32^{+0.20}_{-0.19}$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.00669^{+0.00073}_{-0.00061}$ & $0.002908^{+0.000076}_{-0.000074}$ & $0.00823^{+0.00037}_{-0.00035}$ & $0.01541^{+0.00035}_{-0.00036}$ & $0.00640 \pm 0.00012$ \\
$i$ (deg) & Inclination & $86.85^{+0.76}_{-0.63}$ & $89.20^{+0.56}_{-0.86}$ & $88.6^{+1.0}_{-1.1}$ & $88.11^{+0.13}_{-0.14}$ & $83.68^{+0.26}_{-0.27}$ \\
$K$ (m/s) & RV semi-amplitude & $130 \pm 16$ & $17.3^{+2.8}_{-2.7}$ & $111^{+27}_{-26}$ & $202^{+21}_{-25}$ & $115^{+19}_{-18}$ \\
$a$ (AU) & Semimajor axis & $0.05448^{+0.00085}_{-0.00086}$ & $0.0740^{+0.0013}_{-0.0018}$ & $0.0492^{+0.0009}_{-0.0010}$ & $0.0726^{+0.0013}_{-0.0011}$ & $0.0522^{+0.0008}_{-0.0010}$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $1.303^{+0.069}_{-0.064}$ & $0.974^{+0.025}_{-0.023}$ & $1.281^{+0.044}_{-0.039}$ & $1.101^{+0.041}_{-0.039}$ & $1.191^{+0.040}_{-0.038}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $1.25 \pm 0.16$ & $0.194^{+0.033}_{-0.032}$ & $0.97^{+0.24}_{-0.23}$ & $1.80^{+0.21}_{-0.23}$ & $1.04 \pm 0.17$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.70^{+0.16}_{-0.13}$ & $0.260^{+0.046}_{-0.045}$ & $0.57^{+0.15}_{-0.14}$ & $1.67^{+0.27}_{-0.28}$ & $0.76^{+0.16}_{-0.14}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $3.261^{+0.071}_{-0.076}$ & $2.704^{+0.068}_{-0.079}$ & $3.17^{+0.10}_{-0.12}$ & $3.567^{+0.056}_{-0.069}$ & $3.257^{+0.074}_{-0.082}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.394^{+0.064}_{-0.085}$ & $0.12^{+0.12}_{-0.08}$ & $0.18^{+0.14}_{-0.12}$ & $0.639^{+0.031}_{-0.040}$ & $0.806^{+0.012}_{-0.013}$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & $0.182^{+0.040}_{-0.048}$ & 0.0 (fixed) \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.083$ & $< 0.12$ & $< 0.10$ & -- & $< 0.15$ \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $0.48^{+0.16}_{-0.13}$ & $2.32^{+0.47}_{-0.46}$ & $0.244^{+0.077}_{-0.068}$ & $12.9^{+3.3}_{-2.8}$ & $0.55^{+0.14}_{-0.12}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $1.638^{+0.069}_{-0.064}$ & $1.05^{+0.11}_{-0.09}$ & $1.78^{+0.16}_{-0.14}$ & $0.157^{+0.022}_{-0.019}$ & $1.43^{+0.09}_{-0.11}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1639^{+17}_{-16}$ & $1468^{+36}_{-33}$ & $1673^{+35}_{-33}$ & $919^{+30}_{-29}$ & $1585^{+25}_{-32}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.378^{+0.065}_{-0.064}$ & $1.391^{+0.074}_{-0.097}$ & $1.250^{+0.068}_{-0.075}$ & $0.912^{+0.051}_{-0.040}$ & $1.250^{+0.060}_{-0.072}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.634 \pm 0.046$ & $1.857^{+0.038}_{-0.036}$ & $1.451^{+0.036}_{-0.030}$ & $0.912^{+0.032}_{-0.030}$ & $1.530 \pm 0.041$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.150^{+0.033}_{-0.032}$ & $4.046^{+0.014}_{-0.026}$ & $4.215^{+0.021}_{-0.036}$ & $4.479 \pm 0.034$ & $4.163 \pm 0.027$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.445^{+0.047}_{-0.041}$ & $0.309^{+0.010}_{-0.020}$ & $0.583^{+0.034}_{-0.057}$ & $1.70^{+0.19}_{-0.17}$ & $0.489^{+0.041}_{-0.038}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $3.57 \pm 0.11$ & $4.21^{+0.53}_{-0.43}$ & $3.16^{+0.31}_{-0.27}$ & $0.629^{+0.097}_{-0.082}$ & $2.87^{+0.19}_{-0.25}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $6206^{+90}_{-88}$ & $6070^{+160}_{-150}$ & $6390^{+160}_{-150}$ & $5380^{+180}_{-170}$ & $6060^{+120}_{-140}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $0.216^{+0.089}_{-0.088}$ & $0.288^{+0.076}_{-0.078}$ & $-0.102^{+0.066}_{-0.077}$ & $0.206^{+0.090}_{-0.088}$ & $0.208 \pm 0.078$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $0.299^{+0.080}_{-0.084}$ & $0.316^{+0.077}_{-0.076}$ & $0.039^{+0.056}_{-0.062}$ & $0.208 \pm 0.087$ & $0.247^{+0.069}_{-0.066}$ \\
Age (Gyr) & Stellar age & $2.45^{+0.92}_{-0.84}$ & $3.2^{+1.3}_{-0.8}$ & $2.7^{+1.4}_{-0.9}$ & $8.0^{+3.8}_{-4.1}$ & $4.1^{+1.5}_{-1.1}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $361^{+28}_{-17}$ & $397^{+26}_{-21}$ & $369^{+35}_{-24}$ & $365 \pm 26$ & $401^{+21}_{-30}$ \\
$A_V$ (mag) & Visual extinction & $0.384 \pm 0.020$ & $0.47^{+0.14}_{-0.13}$ & $0.331^{+0.087}_{-0.086}$ & $0.50 \pm 0.21$ & $0.40^{+0.07}_{-0.11}$ \\
d (pc) & Distance & $476.7^{+2.1}_{-2.0}$ & $603.6^{+5.2}_{-5.1}$ & $548.2 \pm 4.4$ & $213.68^{+0.50}_{-0.49}$ & $478.0 \pm 3.2$%
 \\
\multicolumn{\totalcolumns}{c}{\vrule height 24pt width 0pt \small\it\fnum@table\ continued on next page}
\enddata


==> fit_results_5.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \colhead{} & \colhead{TOI-5210\,b} & \colhead{TOI-5322\,b} & \colhead{TOI-5340\,b} & \colhead{TOI-5386A\,b} & \colhead{TOI-5592\,b}
}
\startdata
\multicolumn{7}{l}{\textbf{Planet Parameters}} \\
$P$ (days) & Period & $4.5661061^{+0.0000024}_{-0.0000023}$ & $5.4233207^{+0.0000039}_{-0.0000038}$ & $4.9394392^{+0.0000071}_{-0.0000072}$ & $3.62156552 \pm 0.00000083$ & $2.6085846 \pm 0.0000018$ \\
$T_c$ (BJD$_\mathrm{TDB}$) & Time of conjunction & $2459854.90873 \pm 0.00028$ & $2460035.27909 \pm 0.00030$ & $2459712.57912 \pm 0.00050$ & $2459621.28242 \pm 0.00014$ & $2459794.01216 \pm 0.00032$ \\
$T_{14}$ (days) & Transit duration & $0.1546^{+0.0011}_{-0.0010}$ & $0.2130^{+0.0010}_{-0.0009}$ & $0.2075^{+0.0019}_{-0.0018}$ & $0.09261 \pm 0.00067$ & $0.0827 \pm 0.0013$ \\
$\tau$ (days) & Ingress/egress duration & $0.0123^{+0.0011}_{-0.0007}$ & $0.02044^{+0.00085}_{-0.00032}$ & $0.0187^{+0.0021}_{-0.0016}$ & $0.0380^{+0.0028}_{-0.0021}$ & $0.04136^{+0.00066}_{-0.00065}$ \\
$a/R_\star$ & Planet-star separation & $9.93^{+0.25}_{-0.37}$ & $8.91^{+0.07}_{-0.16}$ & $7.30^{+0.29}_{-0.33}$ & $8.384^{+0.099}_{-0.096}$ & $6.07 \pm 0.21$ \\
$\left(R_P / R_\star\right)^2$ & Transit depth & $0.00662^{+0.00012}_{-0.00010}$ & $0.01086 \pm 0.00011$ & $0.00563^{+0.00013}_{-0.00012}$ & $0.01172^{+0.00027}_{-0.00024}$ & $0.0126^{+0.0052}_{-0.0018}$ \\
$i$ (deg) & Inclination & $88.59^{+0.87}_{-0.75}$ & $89.19^{+0.56}_{-0.68}$ & $86.17^{+0.69}_{-0.73}$ & $83.951^{+0.095}_{-0.094}$ & $81.14^{+0.48}_{-0.68}$ \\
$K$ (m/s) & RV semi-amplitude & $29.7 \pm 4.5$ & $67.0^{+8.9}_{-9.1}$ & $84 \pm 24$ & $58.1^{+5.3}_{-5.1}$ & $116.7^{+7.6}_{-7.7}$ \\
$a$ (AU) & Semimajor axis & $0.0557^{+0.0010}_{-0.0012}$ & $0.0604^{+0.0010}_{-0.0009}$ & $0.0628^{+0.0011}_{-0.0024}$ & $0.04856^{+0.00075}_{-0.00077}$ & $0.03935^{+0.00074}_{-0.00082}$ \\
$R_P$ ($R_\mathrm{J}$) & Planet radius & $0.957^{+0.032}_{-0.024}$ & $1.482^{+0.031}_{-0.027}$ & $1.345^{+0.051}_{-0.049}$ & $1.312^{+0.029}_{-0.028}$ & $1.53^{+0.32}_{-0.16}$ \\
$M_P$ ($M_\mathrm{J}$) & Planet mass & $0.258 \pm 0.041$ & $0.579 \pm 0.081$ & $0.85 \pm 0.25$ & $0.488^{+0.048}_{-0.046}$ & $0.899^{+0.070}_{-0.069}$ \\
$\rho_P$ (g cm$^{-3}$) & Planet density & $0.364^{+0.068}_{-0.067}$ & $0.220^{+0.031}_{-0.033}$ & $0.43^{+0.15}_{-0.13}$ & $0.268^{+0.029}_{-0.028}$ & $0.22^{+0.10}_{-0.12}$ \\
$\log{g_P}$ (cgs) & Planet surface gravity & $2.843^{+0.069}_{-0.081}$ & $2.815^{+0.056}_{-0.066}$ & $3.07^{+0.12}_{-0.15}$ & $2.847^{+0.041}_{-0.043}$ & $2.97^{+0.10}_{-0.19}$ \\
$b \equiv a\cos{i}/R_\star$ & Transit impact parameter & $0.24^{+0.12}_{-0.15}$ & $0.12^{+0.10}_{-0.09}$ & $0.487^{+0.067}_{-0.072}$ & $0.8835 \pm 0.0039$ & $0.941^{+0.033}_{-0.023}$ \\
$e$ & Eccentricity & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) & 0.0 (fixed) \\
$e_\mathrm{lim}$\tablenotemark{a} & 1-$\sigma$ upper limit on eccentricity & $< 0.066$ & $< 0.055$ & $< 0.13$ & $< 0.072$ & $< 0.062$ \\
$\tau_\mathrm{circ}$ (Gyr)\tablenotemark{b} & Tidal circularization timescale & $0.75^{+0.18}_{-0.17}$ & $0.375^{+0.058}_{-0.063}$ & $0.71^{+0.31}_{-0.24}$ & $0.112^{+0.015}_{-0.014}$ & $0.003^{+0.019}_{-0.002}$ \\
$\langle F \rangle$ (Gerg~s$^{-1}$~cm$^{-2}$) & Incident flux & $0.621^{+0.037}_{-0.040}$ & $0.754^{+0.047}_{-0.041}$ & $1.367^{+0.092}_{-0.098}$ & $1.112^{+0.049}_{-0.047}$ & $2.33^{+0.13}_{-0.12}$ \\
$T_\mathrm{eq}$ (K) & Planet equilibrium temperature & $1286^{+19}_{-21}$ & $1350^{+21}_{-19}$ & $1566^{+26}_{-29}$ & $1488 \pm 16$ & $1789^{+25}_{-23}$ \\
\multicolumn{7}{l}{\textbf{Stellar Parameters}} \\
$M_\star$ ($M_\odot$) & Stellar mass & $1.105^{+0.063}_{-0.068}$ & $0.998^{+0.051}_{-0.046}$ & $1.35^{+0.07}_{-0.15}$ & $1.165 \pm 0.055$ & $1.194^{+0.069}_{-0.073}$ \\
$R_\star$ ($R_\odot$) & Stellar radius & $1.209^{+0.032}_{-0.026}$ & $1.462^{+0.028}_{-0.025}$ & $1.842^{+0.055}_{-0.054}$ & $1.245 \pm 0.022$ & $1.393 \pm 0.038$ \\
$\log{g_\star}$ (cgs) & Stellar surface gravity & $4.319^{+0.026}_{-0.040}$ & $4.110^{+0.012}_{-0.018}$ & $4.036^{+0.038}_{-0.056}$ & $4.314 \pm 0.013$ & $4.226 \pm 0.036$ \\
$\rho_\star$ (g cm$^{-3}$) & Stellar density & $0.888^{+0.069}_{-0.095}$ & $0.456^{+0.011}_{-0.024}$ & $0.302^{+0.037}_{-0.039}$ & $0.850^{+0.030}_{-0.029}$ & $0.621^{+0.068}_{-0.061}$ \\
$L_\star$ ($L_\odot$) & Stellar luminosity & $1.42^{+0.08}_{-0.11}$ & $2.03^{+0.12}_{-0.11}$ & $3.94^{+0.25}_{-0.34}$ & $1.927^{+0.075}_{-0.074}$ & $2.64^{+0.12}_{-0.11}$ \\
$T_\mathrm{eff}$ (K) & Stellar effective temperature & $5723^{+95}_{-120}$ & $5692^{+87}_{-83}$ & $5990^{+130}_{-150}$ & $6094^{+67}_{-65}$ & $6237^{+100}_{-96}$ \\
$[\mathrm{Fe/H}]$ (dex) & Metallicity & $0.324^{+0.084}_{-0.086}$ & $-0.048^{+0.042}_{-0.077}$ & $0.208^{+0.081}_{-0.082}$ & $0.182^{+0.093}_{-0.089}$ & $-0.013^{+0.052}_{-0.060}$ \\
$[\mathrm{Fe/H}]_0$ (dex)\tablenotemark{c} & Initial metallicity & $0.326^{+0.075}_{-0.077}$ & $0.015^{+0.049}_{-0.069}$ & $0.243^{+0.083}_{-0.078}$ & $0.203^{+0.080}_{-0.077}$ & $0.080^{+0.050}_{-0.053}$ \\
Age (Gyr) & Stellar age & $5.3^{+3.1}_{-2.3}$ & $9.7^{+2.0}_{-1.8}$ & $3.5^{+2.2}_{-0.9}$ & $3.4^{+1.5}_{-1.2}$ & $3.6^{+1.8}_{-1.4}$ \\
EEP\tablenotemark{d} & Equal evolutionary phase & $397^{+24}_{-38}$ & $446.6^{+5.0}_{-5.7}$ & $405^{+45}_{-24}$ & $372^{+25}_{-26}$ & $387^{+32}_{-38}$ \\
$A_V$ (mag) & Visual extinction & $0.32^{+0.07}_{-0.11}$ & $0.152^{+0.044}_{-0.069}$ & $0.52^{+0.07}_{-0.12}$ & $0.020^{+0.015}_{-0.014}$ & $0.065^{+0.035}_{-0.042}$ \\
d (pc) & Distance & $303.3 \pm 1.5$ & $483.8 \pm 4.1$ & $529.9 \pm 3.6$ & $383.2^{+3.5}_{-3.4}$ & $586.9^{+4.1}_{-4.0}$%
\enddata


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> rv_data.tex <==
% target, bjdtdb, rv, rverr, bis, bis_err, inst
2031 & 2459803.091606 & -32.8 & 7.4 & 64 & 67 & HIRES \\
2031 & 2459828.870264 & 37.8 & 7.4 & -125 & 64 & HIRES \\
2031 & 2459831.950312 & 20.6 & 7.4 & 28 & 65 & HIRES \\
2031 & 2459825.015929 & -69.6 & 7.3 & 21 & 72 & HIRES \\
2031 & 2459833.908365 & 44.2 & 7.7 & -46 & 72 & HIRES \\
2031 & 2459835.049538 & -60.4 & 7.2 & 0 & 69 & HIRES \\
2031 & 2459038.917858 & -335.8 & 68.2 & -- & -- & TRES \\
2031 & 2459058.946837 & -214.8 & 37.3 & -- & -- & TRES \\
2031 & 2459061.967765 & -84.7 & 40.7 & -- & -- & TRES \\
2031 & 2459062.915485 & -125.4 & 49.1 & -- & -- & TRES \\
2031 & 2459071.884140 & 56.6 & 51.7 & -- & -- & TRES \\
2031 & 2459072.823320 & 200.1 & 68.9 & -- & -- & TRES \\
2031 & 2459074.803286 & 84.3 & 52.3 & -- & -- & TRES \\
2031 & 2459075.941391 & 83.2 & 70.2 & -- & -- & TRES \\
2031 & 2459827.047862 & 69.1 & 7.4 & 48 & 70 & HIRES \\
2169 & 2459663.974292 & 12996.1 & 10.4 & -20 & 29 & NEID \\
2169 & 2459081.736184 & 0.0 & 130.1 & -- & -- & TRES \\
2169 & 2459102.653669 & -157.3 & 130.1 & -- & -- & TRES \\
2169 & 2460017.983948 & 13028.4 & 13.0 & 35 & 28 & NEID \\
2169 & 2460012.030361 & 12938.6 & 14.3 & -35 & 46 & NEID \\
2169 & 2460010.004725 & 13241.5 & 34.1 & -- & -- & NEID \\
2169 & 2460037.966461 & 12864.9 & 10.8 & -9 & 27 & NEID \\
2169 & 2460041.000115 & 12952.0 & 10.0 & 13 & 25 & NEID \\
2169 & 2459651.009867 & 12914.4 & 14.6 & -20 & 40 & NEID \\
2169 & 2459737.968454 & 13000.5 & 10.3 & -6 & 22 & NEID \\
2169 & 2460133.893584 & 13010.3 & 11.4 & 32 & 32 & NEID \\
2169 & 2460024.015653 & 12927.4 & 23.1 & -122 & 99 & NEID \\
2169 & 2459679.998833 & 12985.4 & 10.6 & 30 & 31 & NEID \\
2169 & 2459537.581562 & 12859.3 & 12.8 & -43 & 40 & NEID \\
2169 & 2460142.836420 & 12977.3 & 21.3 & -133 & 81 & NEID \\
2346 & 2459832.084142 & -63.9 & 13.1 & 718 & 221 & HIRES \\
2346 & 2459830.090007 & 6.8 & 12.3 & 284 & 174 & HIRES \\
2346 & 2459896.121606 & 199.6 & 12.4 & -325 & 219 & HIRES \\
2346 & 2459897.925766 & -83.7 & 12.3 & -216 & 216 & HIRES \\
2346 & 2459889.994935 & 182.5 & 13.1 & -111 & 127 & HIRES \\
2346 & 2459891.021959 & -32.6 & 13.1 & -140 & 110 & HIRES \\
2346 & 2459896.954979 & 43.8 & 12.2 & -59 & 108 & HIRES \\
2346 & 2459172.897075 & -160.2 & 197.8 & -- & -- & TRES \\
2346 & 2459176.011418 & -968.9 & 157.5 & -- & -- & TRES \\
2346 & 2459184.872116 & -3108.6 & 197.8 & -- & -- & TRES \\
2346 & 2459871.052696 & -155.1 & 13.3 & 357 & 156 & HIRES \\
2346 & 2459835.095118 & -93.1 & 11.8 & 297 & 142 & HIRES \\
2382 & 2459474.665000 & -5522.0 & 39.0 & 23 & 94 & CHIRON \\
2382 & 2459509.556360 & -5459.0 & 46.0 & 2 & 61 & CHIRON \\
2382 & 2459540.569730 & -5353.0 & 31.0 & -9 & 61 & CHIRON \\
2382 & 2459510.578550 & -5524.0 & 41.0 & 120 & 111 & CHIRON \\
2382 & 2459507.595200 & -5386.0 & 58.0 & 120 & 120 & CHIRON \\
2382 & 2459172.621379 & 0.0 & 45.4 & -- & -- & TRES \\
2382 & 2459456.830870 & -5415.0 & 42.0 & 75 & 70 & CHIRON \\
2382 & 2459202.624154 & 59.7 & 45.4 & -- & -- & TRES \\
2382 & 2459546.524380 & -5445.0 & 28.0 & 33 & 52 & CHIRON \\
2382 & 2459570.530860 & -5548.0 & 28.0 & 167 & 136 & CHIRON \\
2382 & 2459508.601250 & -5422.0 & 40.0 & -90 & 80 & CHIRON \\
2382 & 2459542.587740 & -5539.0 & 38.0 & 9 & 74 & CHIRON \\
2382 & 2459460.670400 & -5320.0 & 29.0 & -134 & 65 & CHIRON \\
2876 & 2459958.676450 & 88731.0 & 26.0 & -- & -- & CHIRON \\
2876 & 2459961.693520 & 88718.0 & 39.0 & -- & -- & CHIRON \\
2876 & 2459964.590020 & 88815.0 & 30.0 & -- & -- & CHIRON \\
2876 & 2459985.574595 & -17.4 & 2.9 & -78 & 128 & PFS \\
2876 & 2459897.759583 & -23.7 & 3.4 & -44 & 86 & PFS \\
2876 & 2459983.664155 & 11.5 & 3.1 & -270 & 175 & PFS \\
2876 & 2460046.581215 & 0.4 & 2.4 & 27 & 58 & PFS \\
2876 & 2460072.525926 & 0.0 & 3.6 & 101 & 92 & PFS \\
2876 & 2460064.495231 & -11.8 & 2.3 & 36 & 59 & PFS \\
2876 & 2459532.973398 & -145.7 & 30.7 & -- & -- & TRES \\
2876 & 2459536.908352 & -52.0 & 30.7 & -- & -- & TRES \\
2886 & 2459518.001876 & -53.7 & 24.7 & -- & -- & TRES \\
2886 & 2459534.989030 & 383.9 & 41.6 & -- & -- & TRES \\
2886 & 2459975.747844 & 197.0 & 26.4 & -- & -- & TRES \\
2886 & 2459976.742125 & 175.5 & 28.6 & -- & -- & TRES \\
2886 & 2459977.748087 & -67.2 & 36.3 & -- & -- & TRES \\
2886 & 2459980.823939 & -71.8 & 26.9 & -- & -- & TRES \\
2886 & 2459982.750727 & -277.9 & 51.9 & -- & -- & TRES \\
2886 & 2459984.757276 & 107.5 & 31.5 & -- & -- & TRES \\
2886 & 2459985.747950 & -1.7 & 43.7 & -- & -- & TRES \\
2886 & 2459987.841206 & -24.3 & 34.6 & -- & -- & TRES \\
2886 & 2459991.734341 & 203.4 & 58.7 & -- & -- & TRES \\
2886 & 2460001.788285 & -73.4 & 52.9 & -- & -- & TRES \\
2986 & 2459557.987252 & -80.2 & 43.0 & -- & -- & TRES \\
2986 & 2459585.976754 & 0.0 & 43.0 & -- & -- & TRES \\
2986 & 2459716.643112 & 5358.6 & 6.9 & -15 & 18 & NEID \\
2986 & 2459714.688996 & 5328.1 & 8.1 & 33 & 22 & NEID \\
2986 & 2459732.671328 & 5317.5 & 9.6 & -20 & 44 & NEID \\
2986 & 2459715.697628 & 5291.3 & 9.3 & -22 & 33 & NEID \\
2986 & 2460042.825259 & 5301.6 & 9.0 & 38 & 36 & NEID \\
2986 & 2460014.865755 & 5307.9 & 10.2 & -21 & 44 & NEID \\
2986 & 2460002.870588 & 5339.8 & 13.8 & -46 & 75 & NEID \\
2986 & 2460035.816174 & 5332.0 & 6.7 & 22 & 23 & NEID \\
2986 & 2459709.691400 & 5328.1 & 11.3 & -0 & 47 & NEID \\
2986 & 2460017.869757 & 5299.2 & 9.3 & -64 & 33 & NEID \\
2986 & 2460016.856725 & 5292.6 & 8.8 & 34 & 23 & NEID \\
2986 & 2459739.668003 & 5354.1 & 13.2 & -28 & 63 & NEID \\
2992 & 2459716.507020 & 596.0 & 46.0 & -433 & 221 & CHIRON \\
2992 & 2459683.623520 & 380.0 & 56.0 & 292 & 283 & CHIRON \\
2992 & 2459737.505410 & 555.0 & 77.0 & 163 & 252 & CHIRON \\
2992 & 2459739.543570 & -33.0 & 50.0 & 90 & 137 & CHIRON \\
2992 & 2459738.505540 & -70.0 & 60.0 & 34 & 100 & CHIRON \\
2992 & 2459681.578210 & -229.0 & 66.0 & 264 & 235 & CHIRON \\
3135 & 2459801.494770 & -4803.0 & 66.0 & 32 & 321 & CHIRON \\
3135 & 2459788.528040 & -4924.0 & 63.0 & 240 & 356 & CHIRON \\
3135 & 2459675.683880 & -4708.0 & 82.0 & 245 & 233 & CHIRON \\
3135 & 2459799.511040 & -4972.0 & 78.0 & -106 & 252 & CHIRON \\
3135 & 2459790.501570 & -4610.0 & 125.0 & 92 & 407 & CHIRON \\
3135 & 2459662.781990 & -5023.0 & 59.0 & -165 & 172 & CHIRON \\
3135 & 2459660.809070 & -4740.0 & 46.0 & -121 & 114 & CHIRON \\
3160 & 2459795.518218 & 34.8 & 12.9 & 97 & 319 & PFS \\
3160 & 2459749.655532 & -186.8 & 11.3 & 3 & 135 & PFS \\
3160 & 2459748.688808 & 0.0 & 14.3 & 95 & 137 & PFS \\
3160 & 2459662.880278 & -209.5 & 13.2 & 22 & 90 & PFS \\
3160 & 2459654.830741 & -228.5 & 13.2 & -273 & 184 & PFS \\
3160 & 2459652.809039 & 84.5 & 12.0 & -219 & 111 & PFS \\
3464 & 2459797.511580 & 55346.0 & 56.0 & -77 & 139 & CHIRON \\
3464 & 2459813.541330 & 55098.0 & 26.0 & -131 & 354 & CHIRON \\
3464 & 2460014.846310 & 55005.0 & 41.0 & 32 & 218 & CHIRON \\
3464 & 2460018.823000 & 55079.0 & 57.0 & -8 & 164 & CHIRON \\
3464 & 2460045.799120 & 55260.0 & 57.0 & -5 & 148 & CHIRON \\
3464 & 2459800.514430 & 55258.0 & 51.0 & -256 & 269 & CHIRON \\
3464 & 2460016.890690 & 55218.0 & 50.0 & 53 & 214 & CHIRON \\
3464 & 2460043.798220 & 54839.0 & 78.0 & 99 & 180 & CHIRON \\
3464 & 2460040.818090 & 55047.0 & 74.0 & -1563 & 1603 & CHIRON \\
3474 & 2459795.540160 & -39856.0 & 34.0 & -227 & 120 & CHIRON \\
3474 & 2459793.507200 & -39911.0 & 41.0 & -46 & 85 & CHIRON \\
3474 & 2459817.519030 & -39912.0 & 29.0 & 104 & 88 & CHIRON \\
3474 & 2459811.536970 & -39803.0 & 39.0 & 15 & 119 & CHIRON \\
3474 & 2460012.870870 & -39867.0 & 27.0 & -88 & 103 & CHIRON \\
3474 & 2460013.879120 & -39910.0 & 45.0 & -4 & 105 & CHIRON \\
3474 & 2460023.841410 & -39973.0 & 54.0 & 100 & 103 & CHIRON \\
3474 & 2460044.784310 & -39938.0 & 42.0 & 18 & 113 & CHIRON \\
3474 & 2460051.707160 & -39875.0 & 38.0 & -9 & 130 & CHIRON \\
3474 & 2460022.782320 & -40012.0 & 33.0 & 127 & 76 & CHIRON \\
3474 & 2460057.729570 & -40063.0 & 23.0 & 45 & 125 & CHIRON \\
3486 & 2459793.578380 & -72.6 & 3.8 & -114 & 120 & PFS \\
3486 & 2459749.690451 & 0.0 & 2.6 & 89 & 103 & PFS \\
3486 & 2459795.544560 & -72.5 & 3.3 & -89 & 80 & PFS \\
3486 & 2459796.531898 & 30.4 & 3.5 & -121 & 86 & PFS \\
3486 & 2459828.497616 & -66.4 & 2.5 & 32 & 67 & PFS \\
3486 & 2459450.495430 & 6077.0 & 67.0 & -- & -- & CHIRON \\
3486 & 2459463.517060 & 6080.0 & 57.0 & -- & -- & CHIRON \\
3486 & 2459464.567680 & 6112.0 & 52.0 & -- & -- & CHIRON \\
3486 & 2459827.495671 & 5.5 & 2.7 & 74 & 59 & PFS \\
3523 & 2459838.834802 & 56.1 & 7.5 & -41 & 72 & HIRES \\
3523 & 2459835.849568 & 115.3 & 7.9 & 33 & 158 & HIRES \\
3523 & 2459833.779252 & 157.3 & 7.5 & 143 & 116 & HIRES \\
3523 & 2459431.813581 & -278.8 & 60.5 & -- & -- & TRES \\
3523 & 2459460.687254 & -94.2 & 61.5 & -- & -- & TRES \\
3523 & 2459834.871070 & -208.6 & 7.8 & -109 & 76 & HIRES \\
3523 & 2459829.858884 & -65.1 & 8.5 & -90 & 82 & HIRES \\
3523 & 2459831.932065 & 22.8 & 7.7 & 0 & 77 & HIRES \\
3523 & 2459823.902060 & -79.4 & 8.0 & 178 & 129 & HIRES \\
3593 & 2459791.997889 & 76.4 & 5.3 & 84 & 21 & HIRES \\
3593 & 2459793.016305 & -180.4 & 5.3 & -3 & 37 & HIRES \\
3593 & 2459827.056817 & -148.1 & 5.2 & -29 & 23 & HIRES \\
3593 & 2459829.871142 & 212.1 & 5.3 & 39 & 24 & HIRES \\
3593 & 2459833.918571 & 120.5 & 5.3 & -14 & 24 & HIRES \\
3593 & 2459834.882343 & -182.9 & 5.4 & -21 & 25 & HIRES \\
3593 & 2459460.809585 & -497.4 & 29.8 & -- & -- & TRES \\
3593 & 2459466.687208 & -94.2 & 29.8 & -- & -- & TRES \\
3593 & 2459825.010362 & 167.6 & 5.4 & 42 & 23 & HIRES \\
3593 & 2459831.945502 & -65.7 & 5.2 & -35 & 23 & HIRES \\
3682 & 2459552.902786 & 36076.6 & 9.8 & 89 & 54 & NEID \\
3682 & 2459517.774972 & 36114.0 & 5.1 & 15 & 18 & NEID \\
3682 & 2459561.764753 & 36096.3 & 10.0 & -30 & 37 & NEID \\
3682 & 2459554.906031 & 36120.1 & 6.3 & 32 & 22 & NEID \\
3682 & 2459581.849011 & 36150.8 & 16.6 & -276 & 128 & NEID \\
3682 & 2459572.634985 & 36091.9 & 14.2 & 9 & 92 & NEID \\
3682 & 2459589.844580 & 36062.9 & 9.1 & -55 & 59 & NEID \\
3682 & 2459488.946839 & -94.2 & 40.9 & -- & -- & TRES \\
3682 & 2459476.997048 & 40.3 & 40.9 & -- & -- & TRES \\
3682 & 2459566.900363 & 36066.2 & 9.8 & -4 & 44 & NEID \\
3856 & 2459891.149652 & 79.4 & 5.4 & -2 & 28 & HIRES \\
3856 & 2459896.129350 & -74.2 & 5.4 & -50 & 29 & HIRES \\
3856 & 2459898.062224 & -68.4 & 5.5 & -13 & 29 & HIRES \\
3856 & 2459871.136556 & -6.0 & 5.4 & -24 & 27 & HIRES \\
3856 & 2459890.113845 & -50.6 & 5.3 & 20 & 28 & HIRES \\
3856 & 2460070.915101 & 91.6 & 7.3 & 25 & 69 & HIRES \\
3856 & 2459567.029201 & -390.9 & 35.0 & -- & -- & TRES \\
3856 & 2459567.929894 & -306.1 & 32.1 & -- & -- & TRES \\
3856 & 2459604.996157 & -124.8 & 35.8 & -- & -- & TRES \\
3856 & 2459631.942937 & 25.6 & 5.3 & -6 & 31 & HIRES \\
3856 & 2459654.789054 & 3.7 & 6.1 & 61 & 60 & HIRES \\
3856 & 2459660.976081 & -3.0 & 5.9 & 53 & 166 & HIRES \\
3856 & 2460102.745805 & -12.1 & 5.3 & 179 & 179 & HIRES \\
3877 & 2459584.030099 & 97.9 & 35.1 & -- & -- & TRES \\
3877 & 2459626.869761 & -22.7 & 5.6 & -78 & 78 & HIRES \\
3877 & 2459632.902236 & 25.6 & 5.5 & 93 & 32 & HIRES \\
3877 & 2459661.981852 & 34.6 & 5.6 & -125 & 28 & HIRES \\
3877 & 2459689.978987 & 3.9 & 5.5 & -76 & 28 & HIRES \\
3877 & 2459711.870830 & 20.9 & 5.7 & -3 & 32 & HIRES \\
3877 & 2459738.809049 & -47.8 & 5.6 & 45 & 29 & HIRES \\
3877 & 2459581.994366 & -60.7 & 35.1 & -- & -- & TRES \\
3877 & 2459654.856546 & 23.4 & 5.7 & 136 & 75 & HIRES \\
3877 & 2459742.822874 & -71.0 & 6.0 & 53 & 37 & HIRES \\
3877 & 2459626.069274 & 10.5 & 5.7 & -122 & 41 & HIRES \\
3980 & 2459625.713758 & -42973.8 & 14.4 & -63 & 80 & NEID \\
3980 & 2459552.856891 & -42993.3 & 9.5 & -15 & 33 & NEID \\
3980 & 2459460.974511 & -158.9 & 24.8 & -- & -- & TRES \\
3980 & 2459473.924671 & -94.2 & 24.8 & -- & -- & TRES \\
3980 & 2459538.874350 & -42987.3 & 8.2 & 18 & 23 & NEID \\
3980 & 2459575.609753 & -43001.0 & 12.5 & -19 & 64 & NEID \\
3980 & 2459551.827333 & -43084.9 & 8.2 & -22 & 31 & NEID \\
3980 & 2459597.690973 & -43100.3 & 13.5 & -9 & 59 & NEID \\
4214 & 2459985.582789 & -68.5 & 3.5 & -21 & 68 & PFS \\
4214 & 2460044.586887 & -36.3 & 3.0 & -77 & 62 & PFS \\
4214 & 2460046.589722 & 0.0 & 2.7 & 67 & 85 & PFS \\
4214 & 2460073.486354 & -78.8 & 3.0 & 41 & 63 & PFS \\
4214 & 2460064.485602 & 22.6 & 2.4 & -31 & 43 & PFS \\
4214 & 2459510.817960 & 51599.0 & 48.0 & -- & -- & CHIRON \\
4214 & 2459511.860780 & 51707.0 & 57.0 & -- & -- & CHIRON \\
4214 & 2459513.827520 & 51682.0 & 30.0 & -- & -- & CHIRON \\
4214 & 2459515.818550 & 51659.0 & 24.0 & -- & -- & CHIRON \\
4214 & 2459554.795460 & 51695.0 & 25.0 & -- & -- & CHIRON \\
4214 & 2459559.754440 & 51598.0 & 25.0 & -- & -- & CHIRON \\
4214 & 2459560.744360 & 51609.0 & 32.0 & -- & -- & CHIRON \\
4214 & 2459562.675090 & 51659.0 & 33.0 & -- & -- & CHIRON \\
4214 & 2459564.730920 & 51665.0 & 33.0 & -- & -- & CHIRON \\
4214 & 2459605.640240 & 51571.0 & 26.0 & -- & -- & CHIRON \\
4214 & 2459608.625750 & 51580.0 & 33.0 & -- & -- & CHIRON \\
4214 & 2459610.620290 & 51696.0 & 31.0 & -- & -- & CHIRON \\
4214 & 2459612.624630 & 51566.0 & 28.0 & -- & -- & CHIRON \\
4214 & 2459614.657850 & 51637.0 & 30.0 & -- & -- & CHIRON \\
4214 & 2459616.676220 & 51589.0 & 28.0 & -- & -- & CHIRON \\
4214 & 2459618.595960 & 51631.0 & 35.0 & -- & -- & CHIRON \\
4214 & 2459518.016290 & -52.0 & 37.2 & -- & -- & TRES \\
4214 & 2459526.986417 & 16.6 & 37.2 & -- & -- & TRES \\
4214 & 2459983.672025 & 5.6 & 3.3 & 14 & 67 & PFS \\
4487 & 2459789.937086 & 101.9 & 7.6 & 83 & 124 & HIRES \\
4487 & 2459792.882151 & 83.2 & 8.0 & 48 & 105 & HIRES \\
4487 & 2459776.874612 & 93.7 & 7.5 & 71 & 110 & HIRES \\
4487 & 2459780.062718 & -70.6 & 7.5 & 68 & 70 & HIRES \\
4487 & 2459822.939387 & -115.8 & 8.2 & -171 & 64 & HIRES \\
4487 & 2459776.064195 & -90.0 & 8.2 & 9 & 71 & HIRES \\
4734 & 2459832.104656 & 5.4 & 5.9 & -5 & 46 & HIRES \\
4734 & 2459823.126826 & -8.6 & 5.9 & 2 & 37 & HIRES \\
4734 & 2459834.093584 & 25.0 & 5.8 & 18 & 36 & HIRES \\
4734 & 2459891.040132 & -8.5 & 6.1 & -38 & 34 & HIRES \\
4734 & 2459896.975059 & -3.9 & 6.0 & -33 & 80 & HIRES \\
4734 & 2459890.014551 & 2.3 & 5.9 & -31 & 36 & HIRES \\
4734 & 2459944.906634 & -6.4 & 6.0 & -58 & 39 & HIRES \\
4734 & 2459907.903397 & -15399.9 & 12.6 & 145 & 69 & NEID \\
4734 & 2459936.832838 & -15458.0 & 6.3 & -32 & 16 & NEID \\
4734 & 2459954.797245 & -15395.6 & 11.1 & 34 & 222 & NEID \\
4734 & 2459935.810336 & -15458.1 & 8.2 & 1 & 31 & NEID \\
4734 & 2459952.736089 & -15394.7 & 9.2 & 45 & 144 & NEID \\
4734 & 2460027.715276 & -15440.3 & 13.2 & 55 & 61 & NEID \\
4734 & 2459970.833390 & -15428.3 & 12.0 & -10 & 50 & NEID \\
4734 & 2459953.907693 & -15424.3 & 8.0 & 28 & 24 & NEID \\
4734 & 2459933.822542 & -15426.4 & 7.3 & -7 & 21 & NEID \\
4734 & 2460340.867040 & -15503.8 & 8.0 & -21 & 24 & NEID \\
4734 & 2460327.882889 & -15492.9 & 7.6 & -14 & 30 & NEID \\
4734 & 2460309.936417 & -15498.6 & 9.1 & -23 & 36 & NEID \\
4734 & 2460292.973273 & -15489.6 & 9.7 & -11 & 36 & NEID \\
4734 & 2459586.783254 & 0.0 & 36.7 & -- & -- & TRES \\
4734 & 2459652.701983 & -180.2 & 35.4 & -- & -- & TRES \\
4734 & 2459935.927103 & 1.9 & 36.7 & -- & -- & TRES \\
4734 & 2460037.681388 & -15450.9 & 7.7 & -23 & 30 & NEID \\
4734 & 2459871.058853 & 11.1 & 6.0 & 20 & 37 & HIRES \\
4734 & 2459896.076218 & 12.3 & 5.9 & -43 & 52 & HIRES \\
4734 & 2459943.912378 & -21.6 & 5.9 & -8 & 34 & HIRES \\
4734 & 2459835.081583 & 7.6 & 6.0 & 78 & 87 & HIRES \\
4734 & 2460066.734229 & -47.9 & 6.0 & 80 & 38 & HIRES \\
4794 & 2459969.610680 & 6076.0 & 49.0 & 244 & 177 & CHIRON \\
4794 & 2459965.627590 & 6041.0 & 54.0 & 7 & 149 & CHIRON \\
4794 & 2459967.613380 & 5783.0 & 65.0 & -195 & 137 & CHIRON \\
4794 & 2460002.577780 & 5900.0 & 65.0 & 23 & 157 & CHIRON \\
4794 & 2459985.612080 & 5884.0 & 83.0 & 429 & 248 & CHIRON \\
4794 & 2459988.614010 & 5809.0 & 69.0 & 79 & 240 & CHIRON \\
4794 & 2460017.559320 & 5803.0 & 68.0 & -41 & 282 & CHIRON \\
4794 & 2459963.619170 & 5929.0 & 48.0 & 67 & 226 & CHIRON \\
4794 & 2460014.578520 & 5922.0 & 67.0 & -176 & 173 & CHIRON \\
4794 & 2460044.551330 & 5996.0 & 86.0 & 453 & 198 & CHIRON \\
4794 & 2460060.533740 & 5835.0 & 83.0 & 151 & 157 & CHIRON \\
4794 & 2459592.824259 & -60.7 & 50.5 & -- & -- & TRES \\
4794 & 2459601.828488 & -51.4 & 50.5 & -- & -- & TRES \\
4794 & 2460000.583270 & 5972.0 & 82.0 & -259 & 213 & CHIRON \\
4961 & 2459675.641580 & 25940.0 & 46.0 & -- & -- & CHIRON \\
4961 & 2460043.743472 & -218.3 & 2.8 & -50 & 50 & PFS \\
4961 & 2460045.751285 & 121.9 & 2.8 & 81 & 132 & PFS \\
4961 & 2459984.861007 & -145.0 & 3.0 & 38 & 58 & PFS \\
4961 & 2459988.861782 & 25.6 & 3.1 & -22 & 132 & PFS \\
4961 & 2460072.590683 & -143.2 & 3.0 & -67 & 62 & PFS \\
4961 & 2460047.708646 & 141.8 & 2.8 & 17 & 108 & PFS \\
4961 & 2460067.648727 & 0.0 & 2.9 & -81 & 61 & PFS \\
5181 & 2459740.851667 & 9.5 & 6.7 & -23 & 47 & HIRES \\
5181 & 2459741.914071 & 99.0 & 6.4 & 24 & 46 & HIRES \\
5181 & 2459744.867634 & 22.0 & 6.5 & -14 & 50 & HIRES \\
5181 & 2459738.944248 & -20.4 & 6.3 & 51 & 48 & HIRES \\
5181 & 2459740.015739 & -97.2 & 6.6 & -26 & 46 & HIRES \\
5181 & 2459658.007463 & -206.8 & 38.7 & -- & -- & TRES \\
5181 & 2459663.993316 & -51.4 & 38.7 & -- & -- & TRES \\
5181 & 2459789.772196 & -114.5 & 7.7 & -136 & 108 & HIRES \\
5181 & 2459745.872150 & 101.3 & 6.6 & 159 & 65 & HIRES \\
5210 & 2459781.065020 & 27.0 & 5.6 & -55 & 34 & HIRES \\
5210 & 2459776.833947 & 1.7 & 5.8 & -16 & 37 & HIRES \\
5210 & 2459757.120619 & 4.3 & 6.4 & 58 & 58 & HIRES \\
5210 & 2459702.962189 & -48.0 & 35.1 & -- & -- & TRES \\
5210 & 2459760.125574 & -36.1 & 5.8 & 45 & 32 & HIRES \\
5210 & 2459786.023166 & 11.0 & 5.7 & 2 & 34 & HIRES \\
5210 & 2459766.080723 & 16.0 & 5.6 & -9 & 47 & HIRES \\
5210 & 2459691.962452 & -82.6 & 35.1 & -- & -- & TRES \\
5210 & 2459776.018312 & 20.0 & 5.6 & -52 & 52 & HIRES \\
5210 & 2459768.977731 & -31.2 & 5.7 & -12 & 32 & HIRES \\
5210 & 2459770.085550 & -23.4 & 5.6 & -7 & 32 & HIRES \\
5322 & 2459828.907137 & 22.3 & 5.7 & -29 & 53 & HIRES \\
5322 & 2459829.943490 & -45.3 & 5.8 & -22 & 40 & HIRES \\
5322 & 2459827.078743 & 50.5 & 5.6 & -17 & 40 & HIRES \\
5322 & 2459823.946401 & -14.6 & 5.6 & 56 & 39 & HIRES \\
5322 & 2459832.067965 & 6.5 & 5.7 & 87 & 40 & HIRES \\
5322 & 2459835.021456 & -30.3 & 5.9 & -97 & 103 & HIRES \\
5322 & 2459759.956456 & -126.7 & 34.5 & -- & -- & TRES \\
5322 & 2459767.943907 & -49.3 & 34.5 & -- & -- & TRES \\
5340 & 2459937.876825 & 26365.1 & 25.2 & 137 & 91 & NEID \\
5340 & 2459936.646718 & 26218.8 & 19.4 & -16 & 53 & NEID \\
5340 & 2460011.677981 & 26274.8 & 22.3 & -151 & 122 & NEID \\
5340 & 2459933.885736 & 26353.2 & 21.6 & 1 & 67 & NEID \\
5340 & 2459644.691401 & -186.7 & 68.8 & -- & -- & TRES \\
5340 & 2459804.946223 & 115.7 & 38.2 & -- & -- & TRES \\
5340 & 2459818.928948 & 29.6 & 47.0 & -- & -- & TRES \\
5340 & 2459819.973159 & 17.9 & 37.6 & -- & -- & TRES \\
5340 & 2459820.945112 & -18.5 & 27.5 & -- & -- & TRES \\
5340 & 2459821.958672 & -128.5 & 26.9 & -- & -- & TRES \\
5340 & 2459823.959278 & -20.7 & 44.9 & -- & -- & TRES \\
5340 & 2459824.926317 & 55.1 & 29.8 & -- & -- & TRES \\
5340 & 2459828.950508 & -53.3 & 31.3 & -- & -- & TRES \\
5340 & 2459829.983362 & -7.5 & 27.1 & -- & -- & TRES \\
5340 & 2459833.894103 & 100.2 & 32.3 & -- & -- & TRES \\
5340 & 2459839.961794 & -30.3 & 34.9 & -- & -- & TRES \\
5340 & 2459983.759870 & 26363.7 & 26.4 & 71 & 132 & NEID \\
5386 & 2459775.941266 & 65.1 & 5.3 & -17 & 29 & HIRES \\
5386 & 2459747.819813 & 8.0 & 5.5 & 26 & 42 & HIRES \\
5386 & 2459740.792431 & -0.6 & 5.4 & 75 & 32 & HIRES \\
5386 & 2459771.861633 & 41.0 & 5.4 & 17 & 30 & HIRES \\
5386 & 2459745.836071 & -41.8 & 5.4 & -- & -- & HIRES \\
5386 & 2459744.819161 & -39.9 & 5.5 & 8 & 50 & HIRES \\
5386 & 2459741.794909 & -47.8 & 5.4 & -61 & 36 & HIRES \\
5386 & 2459665.792503 & -149.7 & 46.2 & -- & -- & TRES \\
5386 & 2459674.873705 & -48.0 & 45.9 & -- & -- & TRES \\
5386 & 2460096.748877 & -17491.2 & 7.6 & -- & -- & NEID \\
5386 & 2460066.917453 & -17452.2 & 6.4 & -- & -- & NEID \\
5386 & 2460058.946715 & -17398.9 & 6.7 & -- & -- & NEID \\
5386 & 2460050.984611 & -17385.7 & 5.8 & -- & -- & NEID \\
5386 & 2460032.015503 & -17469.3 & 6.6 & -- & -- & NEID \\
5592 & 2459891.061777 & -117.6 & 6.5 & 43 & 53 & HIRES \\
5592 & 2459898.083167 & 72.1 & 6.6 & 26 & 86 & HIRES \\
5592 & 2459871.086390 & 16.3 & 6.8 & -107 & 107 & HIRES \\
5592 & 2459895.975866 & -64.4 & 6.2 & 185 & 110 & HIRES \\
5592 & 2459953.926646 & -99.0 & 6.9 & -220 & 109 & HIRES \\
5592 & 2459944.934699 & 95.7 & 6.9 & -129 & 114 & HIRES \\
5592 & 2459855.950743 & 236.1 & 42.2 & -- & -- & TRES \\
5592 & 2459864.981170 & -57.6 & 42.2 & -- & -- & TRES \\
5592 & 2459890.075620 & 108.3 & 6.6 & 42 & 59 & HIRES%


==> stellar_companions_0.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \multicolumn{2}{c}{TOI-2031} & \multicolumn{2}{c}{TOI-2169} & \multicolumn{2}{c}{TOI-3160} \\
\colhead{} & \colhead{Primary} & \colhead{Secondary} & \colhead{Primary} & \colhead{Secondary} & \colhead{Primary} & \colhead{Secondary}
}
\startdata
Gaia DR3 ID & 2299101254886404608 & 2299101044431941248 & 4535299582687857920 & 4535299582695351424 & 6225252356194921728 & -- \\
TIC ID & 470127886 & 470127879 & 8516795 & 8516790 & 440872576 & -- \\
Ang. Sep. ($^{\prime\prime}$) & -- & 45.88 & -- & 6.45 & -- & 0.33 \\
Proj. Sep. (AU) & -- & 12820 & -- & 2350 & -- & 160 \\
P.A. ($^{\circ}$) & -- & 148.5 & -- & 233.7 & -- & 348.9 \\
$\mathcal{R}_{\mathrm{chance}}$ & -- & $3.95 \times 10^{-4}$ & -- & $1.89 \times 10^{-5}$ & -- & -- \\
Parallax (mas) & $3.618 \pm 0.013$ & $3.63 \pm 0.11$ & $2.779 \pm 0.017$ & $2.803 \pm 0.014$ & $2.048 \pm 0.037$ & -- \\
$\mu_{\alpha}$ (mas/yr) & $25.790 \pm 0.017$ & $25.76 \pm 0.14$ & $5.505 \pm 0.012$ & $5.270 \pm 0.010$ & $-13.470 \pm 0.038$ & -- \\
$\mu_{\delta}$ (mas/yr) & $2.398 \pm 0.014$ & $2.25 \pm 0.12$ & $-31.042 \pm 0.016$ & $-30.728 \pm 0.016$ & $1.925 \pm 0.035$ & -- \\
RV (km/s) & $-13.69 \pm 0.44$ & -- & $13.09 \pm 0.34$ & $13.4 \pm 1.6$ & $-78.1 \pm 1.6$ & -- \\
$G$ (mag) & $11.1122 \pm 0.0028$ & $18.4108 \pm 0.0031$ & $10.9589 \pm 0.0028$ & $13.6850 \pm 0.0028$ & $12.3656 \pm 0.0028$ & -- \\
$G_\mathrm{BP}$ (mag) & $11.3674 \pm 0.0028$ & $19.981 \pm 0.065$ & $11.2548 \pm 0.0028$ & $14.1640 \pm 0.0030$ & $12.6880 \pm 0.0030$ & -- \\
$G_\mathrm{RP}$ (mag) & $10.6999 \pm 0.0038$ & $17.235 \pm 0.012$ & $10.4951 \pm 0.0038$ & $13.0367 \pm 0.0039$ & $11.8599 \pm 0.0038$ & -- \\
$T$ (mag) & $10.761 \pm 0.036$ & $17.155 \pm 0.013$ & $10.5530 \pm 0.0060$ & $13.1100 \pm 0.0060$ & $11.9330 \pm 0.0070$ & -- \\
AO $\Delta$ mag & -- & -- & -- & -- & -- & \parbox[c][0.75cm][c]{2cm}{\centering 3.30 ($I_c$) \\ $\gtrsim 4$ (832 nm)}%
\enddata


==> stellar_companions_1.tex <==
\tablecolumns{6}
\tablehead{
\colhead{} & \multicolumn{2}{c}{TOI-3464} & \multicolumn{3}{c}{TOI-3523} \\
\colhead{} & \colhead{Primary} & \colhead{Background Star} & \colhead{Primary} & \colhead{Secondary} & \colhead{Tertiary}
}
\startdata
Gaia DR3 ID & 5989042791436795648 & 4531901713810551296 & 2080811118319262080 & -- & 2080811118319127680 \\
TIC ID & 290504044 & 1162931291 & 417047499 & -- & 1971172836 \\
Ang. Sep. ($^{\prime\prime}$) & -- & 2.48 & -- & 0.67 & 8.50 \\
Proj. Sep. (AU) & -- & -- & -- & 410 & 5200 \\
P.A. ($^{\circ}$) & -- & 302.5 & -- & 95.7 & 254.9 \\
$\mathcal{R}_{\mathrm{chance}}$ & -- & -- & -- & -- & $1.24 \times 10^{-2}$ \\
Parallax (mas) & $1.708 \pm 0.013$ & $0.44 \pm 0.21$ & $1.651 \pm 0.029$ & -- & $1.53 \pm 0.20$ \\
$\mu_{\alpha}$ (mas/yr) & $3.716 \pm 0.082$ & $-6.19 \pm 0.45$ & $0.651 \pm 0.031$ & -- & $0.26 \pm 0.21$ \\
$\mu_{\delta}$ (mas/yr) & $-11.814 \pm 0.061$ & $-9.49 \pm 0.30$ & $-12.392 \pm 0.034$ & -- & $-12.60 \pm 0.22$ \\
RV (km/s) & $56.8 \pm 1.7$ & -- & $-4.2 \pm 2.1$ & -- & -- \\
$G$ (mag) & $12.4993 \pm 0.0028$ & $17.9721 \pm 0.0048$ & $12.4966 \pm 0.0028$ & -- & $19.1218 \pm 0.0039$ \\
$G_\mathrm{BP}$ (mag) & $12.8295 \pm 0.0028$ & $17.080 \pm 0.061$ & $12.7583 \pm 0.0029$ & -- & -- \\
$G_\mathrm{RP}$ (mag) & $12.0015 \pm 0.0038$ & $16.324 \pm 0.063$ & $12.0166 \pm 0.0038$ & -- & -- \\
$T$ (mag) & $12.0720 \pm 0.0060$ & $17.440 \pm 0.020$ & $12.104 \pm 0.022$ & -- & $18.71 \pm 0.60$ \\
AO $\Delta$ mag & -- & \parbox[c][1cm][c]{2cm}{\centering 5.50 ($I_c$)} & -- & \parbox[c][1cm][c]{2cm}{\centering 2.058 ($H$cont) \\ 2.105 (Br$\gamma$) \\ 3.5 ($I$)} & --%
 \\
\enddata


==> stellar_companions_2.tex <==
\tablecolumns{7}
\tablehead{
\colhead{} & \multicolumn{2}{c}{TOI-4487} & \multicolumn{2}{c}{TOI-5181} & \multicolumn{2}{c}{TOI-5386} \\
\colhead{} & \colhead{Primary} & \colhead{Secondary} & \colhead{Primary} & \colhead{Secondary} & \colhead{Primary} & \colhead{Secondary}
}
\startdata
Gaia DR3 ID & 2083061376251298688 & 2083061371948751616 & 4531901709506539776 & 4531901713810551296 & 1616054670018575872 & -- \\
TIC ID & 193754373 & 193754364 & 346667887 & 1813596259 & 202425357 & -- \\
Ang. Sep. ($^{\prime\prime}$) & -- & 6.93 & -- & 1.65 & -- & 0.24 \\
Proj. Sep. (AU) & -- & 3360 & -- & 790 & -- & 90 \\
P.A. ($^{\circ}$) & -- & 356.7 & -- & 172.5 & -- & 240.6 \\
$\mathcal{R}_{\mathrm{chance}}$ & -- & $5.44 \times 10^{-4}$ & -- & $3.53 \times 10^{-4}$ & -- & -- \\
Parallax (mas) & $2.0972 \pm 0.0091$ & $2.18 \pm 0.20$ & $2.090 \pm 0.014$ & $2.43 \pm 0.12$ & $2.608 \pm 0.024$ & -- \\
$\mu_{\alpha}$ (mas/yr) & $-0.570 \pm 0.010$ & $-0.78 \pm 0.23$ & $8.3480 \pm 0.0090$ & $8.38 \pm 0.15$ & $-16.116 \pm 0.029$ & -- \\
$\mu_{\delta}$ (mas/yr) & $-13.500 \pm 0.010$ & $-13.65 \pm 0.22$ & $2.698 \pm 0.012$ & $3.63 \pm 0.12$ & $6.295 \pm 0.028$ & -- \\
RV (km/s) & $-10.26 \pm 0.77$ & -- & $-13.51 \pm 0.56$ & -- & $-16.40 \pm 0.47$ & -- \\
$G$ (mag) & $11.9204 \pm 0.0028$ & $19.2344 \pm 0.0044$ & $12.2091 \pm 0.0028$ & $17.2894 \pm 0.0034$ & $11.7564 \pm 0.0028$ & -- \\
$G_\mathrm{BP}$ (mag) & $12.2474 \pm 0.0028$ & $19.90 \pm 0.13$ & $12.5907 \pm 0.0028$ & -- & $12.0559 \pm 0.0028$ & -- \\
$G_\mathrm{RP}$ (mag) & $11.4284 \pm 0.0038$ & $17.893 \pm 0.023$ & $11.6558 \pm 0.0038$ & -- & $11.2883 \pm 0.0038$ & -- \\
$T$ (mag) & $11.492 \pm 0.016$ & $18.420 \pm 0.037$ & $11.7240 \pm 0.0090$ & $16.64 \pm 0.60$ & $11.3500 \pm 0.0070$ & -- \\
AO $\Delta$ mag & -- & -- & -- & \parbox[c][1.25cm][c]{2cm}{\centering 4.51 (832 nm) \\ 4.40 ($I$) \\ 3.015 (Br$\gamma$) \\ 3.179 ($H$cont)} & -- & \parbox[c][1.25cm][c]{2cm}{\centering 1.784 (Br$\gamma$) \\ 2.071 ($H$cont)}%
\enddata

